Database Reconstruction from Noisy Volumes: A Cache Side-Channel Attack on SQLite

We demonstrate the feasibility of database reconstruction under a cache side-channel attack on SQLite. Specifically, we present a Flush+Reload attack on SQLite that obtains approximate (or "noisy") volumes of range queries made to a private database. We then present several algorithms that, taken together, reconstruct nearly the exact database in varied experimental conditions, given these approximate volumes. Our reconstruction algorithms employ novel techniques for the approximate/noisy setting, including a noise-tolerant clique-finding algorithm, a "Match & Extend" algorithm for extrapolating volumes that are omitted from the clique, and a "Noise Reduction Step" that makes use of a closest vector problem (CVP) solver to improve the overall accuracy of the reconstructed database. The time complexity of our attacks grows quickly with the size of the range of the queried attribute, but scales well to large databases. Experimental results show that we can reconstruct databases of size 100,000 and ranges of size 12 with error percentage of 0.11 % in under 12 hours on a personal laptop.

==> Database Cache Attack/attack.tex <==
\section{Our Attack}\label{sec:attack}

\iffalse
In this section we will present our end-to-end attack.
Specifically, we will describe how the cache attack is launched on SQLite to obtain the approximate/noisy volumes. Once the noisy volumes are found, an instance of the noisy clique finding problem will be created, whose solutions correspond to approximately reconstructed candidate databases. The graph must be crafted carefully, since the obtained volumes
are noisy and so naive methods for forming the clique-finding instance will lead to situations where 
no solution exists or too many candidate solutions exist. 
%the maximum clique found is too small
%to allow for even approximate reconstruction.
%the size of the cliques are much smaller than the potential candidate database and their size are so small than they can not be combined to form larger clique. 
\dnote{Perhaps: ``No solution exists or too many candidate solutions exist.''}\anote{tried to address}
%In order to form an instance of the problem we have to note that obtained volumes are noisy and as a result we have to construct an instance in a specific way. The solver then output an answer indicating the potential database. 
However, as we will show in some of the cases, just running the clique finding algorithm cannot recover the original database. In those cases we present a novel algorithm called Match \& Extend to reconstruct the database.
\dnote{Mention Explain algorithm here as well.}\anote{added the previous sentence for this}

Once we have recovered solutions to the clique-finding instance that are somewhat close to the correct solution, we can improve the quality of the solution even further by exploiting the additional structure of the problem. Namely, in a ``correct'' solution the volume of any range $[i-j]$ can be expressed as a linear combination of the volumes of the ranges $[1-1], [2-2], \ldots, [N-N]$.
Hence we craft an instance of the closest vector problem (CVP) on lattices. The solution to the CVP problem will yield a candidate database that is even closer to the real database.
\fi

%\dnote{This is not up-to-date!!}\anote{fixed}
In Section~\ref{sec:aprox_vol} we describe how to recover approximate volumes via the cache side-channel.
%In Section~\ref{sec:subgraph_iso_noiseless} we begin with a warm-up describing how subgraph isomorphism can be used to solve the database reconstruction problem, given \emph{exact} volumes for all ranges.
In Section~\ref{sec:clique} we describe how the clique-finding algorithm was used in the prior work of Grubbs et al.~\cite{grubbs2018pump} to recover a database from noiseless volumes. In Section~\ref{sec:noisy_clique} we explain our noise-tolerant clique-finding algorithm for our setting, where volumes are noisy. In Section~\ref{sec:match_extend} we present the details of the Match \& Extend algorithm which is used for extrapolating volumes that are omitted from the clique.
%to give enhance the performance in cases where just clique-finding was not successful. 
Finally in Section~\ref{sec:CVP} we describe how to use
closest vector problem (CVP) solvers to further reduce the noise and improve the overall accuracy of the recovered databases.



%\anote{here} and \ref{sec:CVP}, we describe how subgraph isomorphism and CVP can be used to solve the database reconstruction problem, given \emph{noisy} volumes. The procedures described in Sections~\ref{sec:subgraph_iso_noisy} \anote{here} and \ref{sec:CVP} constitute our main attack. In Sections~\ref{sec:aux_query} \anote{here} and \ref{sec:aux_data} \anote{here} we describe variants of our main attack that incorporates auxiliary information about either the query distribution or the data distribution into the subgraph isomorphism instance. \mnote{is this up-to-date? I don't remember such a thing} Finally, in Section~\ref{sec:efficient} \anote{here} , we discuss techniques for reducing the complexity of the attack.

\subsection{Recovering Approximate Volumes}\label{sec:aprox_vol}
%\anote{explain the cache recovery part}

%\dnote{Are you now discussing the BTree data structure at some point?}\anote{I have added that in the followng section after ``Detecting Lines to Monitor''}

In this section, we explain how to find the lines of code in the SQLite library to monitor in the Flush+Reload attack and how to reduce the noise in our measurements. We will then explain how to recover the approximate volumes. 

%\vspace{-3mm}

\paragraph{Victim's Query} The victim issues a range query to SQLite database. SQLite returns the relevant entries as it processes the query. These entries are simply saved in a linked list and once SQLite is finished with processing the query, 
%\mnote{what does it mean ``response to the query is completed''?}\anote{fixed}
the linked list is returned to the victim.

%\anote{mention the linked list}\anote{added}

%\vspace{-3mm}

\paragraph{Detecting Lines to Monitor}
SQLite stores columns using the BTree data structure.
We examined the SQLite program, and by using the \texttt{gcov} command we detected lines that are called once in each iteration of a range query. Monitoring the number of times these lines are called allowed us to determine the volume of a query response.
%We are looking for the lines which leak the volume of the query response. 
It is important to notice that the duration of each query can also be measured and that can also be used as an indicator for the volume. However, this resulted in far greater noise since there was no reliable way to translate time to volume (time to iterate over rows was inconsistent). Hence we decided to explicitly count.
To obtain the number of times each line is executed we compiled our library using \texttt{-fprofile-arcs} and \texttt{-ftest-coverage} flags.
%as is shown in lines 1-3 of the Figure~\ref{fig:compile_syntax}. In Line 4 of Figure~\ref{fig:compile_syntax},
We ran the range query command and by using the \texttt{gcov} command 
%in Lines 5 and 6  
we counted the number of times each line is executed in files sqlite3.c and main.c, respectively. 
%The remaining lines gives an .html format of the output to better interpret the results. 

\iffalse
\begin{figure}
    \centering
    \scriptsize
    \begin{lstlisting}[style=CStyle]
    gcc -c -fPIC sqlite3.c -g -fprofile-arcs -ftest-coverage -L /usr/lib -I /usr/include
    gcc -shared -o libsqlite3.so -fPIC sqlite3.o -g -fprofile-arcs -ftest-coverage -L /usr/lib -I /usr/include
    gcc main.c libsqlite3.so -o main -lpthread -ldl -g -fprofile-arcs -ftest-coverage -L /usr/lib -I /usr/include
    ./main db "Select * From TABLE Where COLUMN Between 1 AND 8"
    gcov sqlite3.c 
    gcov main.c 
    lcov -c -d . -o main_coverage.info
    genhtml main_coverage.info --output-directory out
    \end{lstlisting}
        \caption{Compiling and running the SQLite using \texttt{gcov}}
        \label{fig:compile_syntax}
\end{figure}
\fi

\iffalse
\begin{figure}
 \centering
  \includegraphics[width=\linewidth]{figures/gcov_output.png}
  \caption{The output of \texttt{gcov} which is being used to detect what lines can be monitored. In this specific example the range query had to return $1000$ entries from the database and the lines between line 71252 and line 71262 were executed $1000$ times.
  }
  \label{fig:gcov_output}
\end{figure}

A snapshot of the output file is shown in Figure~\ref{fig:gcov_output}. In this specific example the range query returned $1000$ records. We can potentially monitor any of the lines between line $71252$ and line $71262$.
\fi

We looked for more lines throughout the SQLite\footnote{The attack presented in this paper can be extended to other database management system, as long as the volume of the returned query can be obtained through monitoring the I-cache.} program and we chose to simultaneously monitor \emph{two} lines to increase the measurement accuracy. 
As also observed by Allan et al.~\cite{allan2016amplifying}, monitoring two lines has the benefit that in case the attack code fails to detect an activity in one of the lines due to overlap between attacker reload and victim access \dnote{due to ***}\anote{addressed} there is still a high probability of seeing activity in the second line. There might be some excessive false positives due to the mismatch of hits for both of the lines and we mitigate for that by considering close hits to be from the same activity. 
\dnote{I remember that monitoring two lines can also cause false positives. Can you discuss how you detected/removed the false positives.}\anote{done}





%We detected a couple more instances throughout the database file. 

%\vspace{-3mm}

\paragraph{Using the Mastik Toolkit.}
Once we detect the lines that leak the volume of the queries, we use the Mastik Toolkit to monitor those lines while SQLite is processing a range query. 

\iffalse
The following is the command we use to monitor the lines.

\begin{figure}
    \centering
    \begin{lstlisting}[style=CStyle]
    Mastik-0.02-AyeAyeCapn/demo/FR-trace -s 5000 -c 20000000 -h 100 -i 5000 -f libsqlite3.so -m "sqlite3.c:71262" -m "sqlite3.c:80417" > Traces/trace_1.txt
    \end{lstlisting}
    \caption{Parameter set for Mastik}
    \label{fig:mastik_param}
\end{figure}

\dnote{The following itemized list can probably be removed since we are short on space...}
We explain how we set each flag for the \texttt{FR-frace} program. 
\begin{itemize}
    \item \texttt{-s}: is the \texttt{SLOT} flag which is the time we wait after flushing a line before we reload that line again. It has to be set large enough so that we detect a victim activity in the wait time and not so long that victim does two cache accesses during the wait time. 
    \item \texttt{-c}: is the \texttt{SAMPLES} flag that is the maximum number of samples in the trace. It has to be set large enough that the largest volume can be detected. 
    \item \texttt{-h}: is the \texttt{THRESHOLD} flag, any timing value greater than this is considered a cache miss.
    \item \texttt{-i}: is the \texttt{IDLE} flag, which sets the number of inactive samples that should cause the measurement to end. For our case we set it to some large value such that if there is an inactive period during the query execution, the trace doesn't end prematurely. 
    \item \texttt{-f}: is the \texttt{FILE} flag, is the file we are tracking. We are in the shared library setting so we are tracking the Shared Object file.
    \item \texttt{-m}: is the \texttt{MONITORED} flag, that is the lines we are monitoring. We are monitoring two lines.
\end{itemize}
\fi

\iffalse
\begin{figure}
 \centering
  \includegraphics[width=0.8\linewidth]{figures/cache_activity2.pdf}
  \caption{The result of running Flush+Reload attack on SQLite. There are two lines being monitored by attacker. The x-axis shows the sample point in which reload occurs and y-axis depicts the amount of time needed to reload monitored line from memory at that time instance. Since two lines are being monitored, we have two sets of measurement at each time instance. The ``range query execution'' shows the time interval in which SQLite program is executing the range query hence there are some activity in the monitored lines. The ``no activity'' period shows the time in which the SQLite program was not executing the lines which we were monitoring.}
  \label{fig:cache_activity}
\end{figure}
\fi

Figure~\ref{fig:trace_details} shows one sample measurement. Two monitored lines are represented by blue and orange color. Mastik-\texttt{FR-trace} will automatically start measuring once it detects a hit in either of the monitored lines in the SQLite program. 
%In the figure the marked area shows where the range query is being executed. 
Once there is no more activity detected by Mastik for a while (as set in the \texttt{\small IDLE} flag), it will automatically end the measurement. During the interval where range query execution occurs, there are samples with reload time less than $100$ cycles. Those are the samples points in which SQLite accessed the line the attacker is monitoring and hence a small reload time is seen by the attacker. We then count the number of times there is a hit in either a blue or orange measurement. 
%\mnote{don't we count the times both blue and orange have hits?}\anote{not really}. 
The hit count corresponds to the volume of the query. 
\begin{figure}
 \centering
  \includegraphics[width=0.8\linewidth]{figures/sample_trace.pdf}
  \caption{The result of running Flush+Reload attack on SQLite. There are two lines being monitored by attacker. The x-axis shows the sample point in which reload occurs and y-axis depicts the amount of time needed to reload the monitored line from memory at that time instance. Since two lines are being monitored, we have two sets of measurement at each time instance. Notice there are some orange lines appearing close to each other, those are because of speculative execution.}
  \label{fig:trace_details}
\end{figure}

Monitoring the relevant cache lines is also crucial to detect when/if range queries are issued. Figure~\ref{fig:query_activity} shows the cache activity of three cache lines in the first couple of thousands of samples. The cache line activity represents the number of hits detected by the attacker. Counting the number of hits represents whether or not the victim is using a specific line. We expect to see multiple cache activities in lines related to range queries and for the queries that are not relevant to range queries there is not much activity going on in at least one of the cache lines.

\iffalse
\begin{table}[]
\caption{TBD}
\footnotesize
\begin{tabular}{|l|c|}
\hline
\multicolumn{1}{|c|}{Query Name} & Number of hits(min-max) \\ \hline
SELECT DISTINCT & 1-8 | 0-0 | 14-107 \\ \hline
ORDER BY & 1-340 | 0-0 | 0-2 \\ \hline
COUNT & 1-2 | 0-0 | 1-1 \\ \hline
AVERAGE  & 1-17421 | 0-17835 | 0-7 \\ \hline
MIN-MAX & 0-50 | 0-2 | 0-4\\ \hline
GROUP BY & 1-1 | 1-1 | 2-2\\ \hline
RANGE QUERY & - \\ \hline
\end{tabular}
\label{tab:querycount}
\end{table}
\fi

\begin{figure}[t]
 \centering
  \includegraphics[width=0.8\linewidth]{figures/query_activity.pdf}
  \caption{Cache line activity when different queries are issued. The cache line activity represents the number of hits detected by the attacker. The figure is in log scale. It can be seen that by looking at the cache activity of these three lines, different queries can be distinguished.}
  \label{fig:query_activity}
\end{figure}

%\vspace{-3mm}

\paragraph{Noise in the traces}
The number of hits that we count might be different than the actual value of the volume since measurements are not noiseless. Here we explain some of the sources of noise. 
\begin{itemize}
    \item False Positive: Speculative execution of an instruction causes the memory line to be brought into the cache \emph{before} it is executed. In terms of the Flush+Reload attack, it will still \emph{look like} this instruction was executed, since there will be a fast access. Generally the true hits happen at fixed time intervals. If we see a hit which happens much sooner than the expected time for a hit it is most likely a false positive and we assume it occurred due to speculative execution and do not count it as a hit.
    \item False Negative: These occur if the victim process accesses the monitored line of code after the spy \emph{Reloads} the line, and before the spy
    \emph{Flushes} the line. 
    We do not attempt to detect false negatives experimentally, but rather deal with them algorithmically: as will be discussed in Section~\ref{sec:noisy_clique}, we use an asymmetric window around each observed volume to compensate for the fact that true volumes are typically greater than the observed volume. In our experiments we allocate $90 \%$ of the window width to the values greater than the observed volume. 
\end{itemize}

%There are some traces which is considered to be noisy. After going over some traces which was not good enough, we decided to drop traces if either of the two scenarios occurs (a) There are multiple zeros in the measurement which indicated that Mastik was not successful in measuring time at those sample points (b) There is a huge gap in the measurements which could potentially means that Mastik misses couple of samples. 

%\vspace{-3mm}

\paragraph{Running the experiment}
We randomly select 
%a lower bound $a$ and an upper bound $b$ and 
and
execute range query $[a,b]$ while concurrently monitoring lines using Mastik-\texttt{FR-trace} to gather a single trace. We repeat this experiment a number of times in order to gather enough traces. For each trace we count the number of times that either of the lines shows a hit and after mitigating the False Positive issue, we report the number of hits as the volume of the range query for that trace.  

Figure~\ref{fig:volume_attack} shows the result of aggregating the volumes reported by the traces. Some volumes are observed far more frequently than others, and those values are saved as an approximation to the expected volumes.
%We select the values from this figure which occur more than a certain threshold amount (which is selected heuristically by observing the figure).
In a noiseless setting we expect to see at most $\binom{N}{2} + N$ values (there might be some volumes which correspond to more than one range query). In the noisy setting, there are cases where the trace is ``good enough'' but the volume is not correct. By aggregating all the traces the effect of those instances will be insignificant and the approximation of correct volumes will stand out. However, the volumes we recover are not exactly the correct volumes from the database.
\begin{figure}[h]
 \centering
  \includegraphics[width=0.8\linewidth]{figures/volume_attack2.pdf}
  \caption{Sample noisy volumes recovered by cache attack. The x-axis is the volume and y-axis shows the number of occurrence of that volume. For a sample database, we ran the range query multiple times and for each range query we monitored the cache activity to recover the volume of the range for that query. We repeated this process multiple times and counted how many times a volume occurred.  
  %\dnote{A reader should be able to look at the figure only and understand what is going on from the caption. So in the caption you need to specify, what is the x axis, what is the y axis. How were these volumes obtained? E.g. you generated a database in some way, then ran the cache attack some number of times, etc.}
  }
  \label{fig:volume_attack}
\end{figure}
Figure~\ref{fig:aprox_vs_real} shows a closer snapshot of Figure~\ref{fig:volume_attack} for volumes in the range $7700-8800$. The red dotted bars represent the actual volume of the range query response, while the blue line shows the approximate volumes recovered by the cache attack. For every correct volume (red line), there is a blue line with some high value close to it. 

\begin{figure}
 \centering
  \includegraphics[width=0.8\linewidth]{figures/aprox_vs_real.pdf}
  \caption{A closer look at the recovered volumes. The blue figure is the actual measurement from processing traces from the cache attack. The red bar is the actual volume expected to be observed. It can be seen that the recovered volumes (blue) is approximate version of actual volumes (red).}
  \label{fig:aprox_vs_real}
\end{figure}



\subsection{Clique Finding--Noiseless Volumes}\label{sec:clique}

To construct the graph we first explain the clique finding algorithm of Grubbs et. al.~\cite{grubbs2018pump} and then extend their technique to cover the noisy case. There are two main parts to the Algorithm. 
\begin{itemize}
    \item \textbf{Creating Nodes} Given the set of recovered volumes $V$ we create a node for representing each volume and label the node by its corresponding volume, meaning the node $v_i$ has volume $v_i$. 
    \item \textbf{Creating Edges} We create an undirected edge between two nodes $v_i, v_j \in V$ if there exists a node $v_k \in V$ such that $v_i = v_j + v_k$. 
\end{itemize}

By running the clique finding algorithm on the constructed graph, one can recover the volumes. Assuming the range of values are from $1$ to $N$ there are $\binom{N}{2} + N = \frac{N(N+1)}{2}$ possible ranges, and therefore $\frac{N(N+1)}{2}$ nodes in the graph. 
Each range $\range{i}{j}$ for $1 \leq  i \leq j \leq N$ is represented by a node. The nodes that correspond to ranges of the format $\range{1}{i}$ for $1 \leq i \leq N$, i.e. elementary volumes, form a clique, since for each pair of ranges of the form $\range{1}{i}$ and $\range{1}{j}$ for $1 \leq i < j \leq N$ there is another range of the form $\range{i+1}{j}$ %\mnote{should this be (i+1)-j?}\anote{fixed} 
for $1 \leq i < j \leq N$, which implies, due to how the graph is constructed, that there is an edge between 
$\range{1}{i}$ and $\range{1}{j}$.
The clique finding algorithm finds the nodes $\range{1}{i}$ for $1 \leq i \leq N$. To recover the original ranges which are of the form $\range{i}{i}$ for $1 \leq i \leq N$, all that is needed is to sort the nodes based on their labels, which corresponds to their volumes, and subtract them sequentially since $\size{\range{i}{i}} = \size{\range{1}{i}} - \size{\range{1}{i-1}}$ for $1 < i \leq N$. 
\iffalse
\dnote{Is the next sentence relevant?}\anote{moved this from the next subsection and reword it} \mnote{the next sentence feels out of nowhere}\anote{I think we can get rid of the following sentence all together} 
This approach is often effective to recover the original database given the volumes but even in the noiseless setting of Grubbs et. al.~\cite{grubbs2018pump}, note that there were some databases that could not be fully recovered via their clique-finding method.
%\footnote{The main algorithm has a prepossessing step and after that clique finding is applied \dnote{I don't understand this footnote.}}. 
\fi

%\vspace{-3mm}
\subsection{Clique Finding--Noisy Volumes}\label{sec:noisy_clique}
In the noisy case considered here, all recovered volumes are close to the correct volumes, but the exact volumes may not have been recovered. 
Hence, the procedure for noiseless case fails to find the cliques of large enough size. This is because the condition to connect 
nodes $v_i, v_j$ will almost always fail
(even when there should be an edge)
since there will not be a third volume $v_k$ such that the equation $v_i = v_j + v_k$ is exactly satisfied. 
This means that the constructed graph is missing too many edges and the large cliques are not formed. 
To mitigate the effect of the noise, we modify the second step of the graph generation algorithm i.e. \textit{Creating Edges}. 

%In the following we explain the idea behind the algorithm and how it works. 

While the recovered volumes are close to the correct ones, as explained in Section~\ref{sec:aprox_vol}, since the traces are noisy we do not expect to get the exact volumes and we often under-count.
%\mnote{should we say "we often under-count, but in a predictable manner" and then say something about the measurements being close to some number away from real volumes?}\anote{addressed in False NEgative}
We call the ratio of the recovered volume to the correct volume the ``noise ratio''. In the first step the attacker performs a preprocessing step which involves mounting the attack on a database known to the attacker. The attacker then assesses the quality of the traces to find the approximate value of the ``noise ratio''. To find it the attacker heuristically looks at the recovered volumes and compares them to the correct volumes they are expecting to compute. Then based on all the noise ratios, the attacker sets a value for ``noise budget'' which is the mean of the 
%\mnote{not exactly the maximum, more like the mean or the mode i think}\anote{fixed} 
``noise ratio'' he observed over all volumes. Once the noise budget is fixed, for each recovered volume the attacker creates a window of acceptable values around it. Assuming the recovered volume is $v_i$, the attacker creates an asymmetric window around $v_i$ with lower bound and upper bound of $v_i \times (1 - 0.1 \cdot \texttt{\small noise budget})$ and $v_i \times (1 + 0.9 \cdot \texttt{\small noise budget})$, respectively. As also mentioned in Section~\ref{sec:aprox_vol}, the window is asymmetric with $90\% $ of its width on the right hand side of it, as the noisy volumes are typically less than the true volumes.
%due to false positives.  
For a volume $v_i$ we denote by $w(v_i)$ the window around it. To construct the graph in the noisy case we modify the second step of the algorithm explained in Section~\ref{sec:clique} as follows: 

\begin{itemize} 
    \item \textbf{(Modified) Creating Edges} We create an undirected edge between two nodes $v_i \in V$ and $v_j \in V$ if there exists a node $v_k \in V$ such that $| v_i - v_j | \in w(v_k)$. 
\end{itemize} 

In particular, we will say that candidate volumes $u$ and $v$ are ``approximately equal'' if $\frac{|u-v|}{min(u,v)} \le \texttt{\small noise budget}$. As we will show in Section~\ref{sec:experiments}, using the above algorithm with the just-mentioned modification 
%\mnote{"...using the above algorithm with the just-mentioned modification..."?}\anote{added} 
is in some cases sufficient to approximately reconstruct the database.

%\vspace{-3mm}
\subsection{Match \& Extend}\label{sec:match_extend}

In this section we describe an improvement on the noisy clique-finding algorithm that is used in cases where the noisy clique-finding algorithm fails to find a maximal clique of size $N$, even with appropriate adjustment of the noise budget. 
%Our final goal is to consider the case in which the volumes are approximate and there is no clique of size $N$ present in the noisy graph. For the purpose of describing our algorithm, in the following we will first present an example.

%first consider the case where the volumes are exact (noiseless) but a volume of some range query is \emph{missing}.

First, recall that the idea behind the clique finding algorithm is that if we have the volumes of all ranges present in our data, then there must exist a clique in the graph corresponding to the volumes of the ranges $\range{1}{i}$ for $1 \leq i \leq N$. Now, let us assume there is a missing (approximate) volume corresponding to range $\range{i}{j}$.  This will result in the missing connection from the node $\range{1}{j}$ to node $\range{1}{i-1}$ as the reason that there had to be a connection was because $\size{\range{1}{j}} \approx \size{\range{1}{i-1}} + \size{\range{i}{j}}$. As a result of this missing volume, the maximal clique of size $N$ will not form. If we run the clique finding algorithm on the data with the missing volume, it will return cliques of size smaller than $N$ and for each of them recover a candidate database. Then the algorithm will merge the information in these smaller databases to form larger ones. In the following we explain the idea of the algorithm with an example.
Consider a database with $5$ possible values in the range, i.e. $N = 5$, assume the database is $\mydb{30, 100, 80, 30, 60}$ (i.e.~the database contains $30$ records with value $1$, $100$ records with value $2$, etc.). The set of possible values for the volume of a range query is $V = \{30, 60, 80, 90, 100, 110, 130, 170, 180, 210, 240, 270, 300\}$, i.e. $\size{\range{1}{1}} = 30$, $\size{\range{1}{2}} = 130$ and so on. The graph constructed from the these volumes is shown in Figure~\ref{fig:clique1} and the maximal clique found by the clique finder algorithm is shown by bold connections.
The returned nodes are $\{30, 130, 210, 240, 300\}$ and the reconstructed database is $\mydb{30, 100, 80, 30, 60}$.
Assume the recovered volumes are noisy and the set of possible values for the volume of a range query is $V = \{29, 58, 79, 89, 98, 108, 128, 160, 178, 209, 239, 268, 299\}$. 
In Figure~\ref{fig:clique2} all the noisy volumes are rather close to their actual values except the volume $160$ which is far from the correct one --- $170$. 
To construct the graph in this setting we use the algorithm mentioned in Section~\ref{sec:noisy_clique} and only for the sake of this example we take the window around volume $v_i$ to have lower and upper bound of $v_i - 1$ and $v_i + 3$, respectively. 
%The volume and all it's connection to the rest of the graph will be missing as a result of missing that volume. There are also other connections missing. 
Some connections will be missing as a result of the error in the measurement. For example the connection from node $299$ to node $128$ is not going to be formed since there is no longer a window which contains $171$. If we run the clique finding algorithm on the new graph the result is going to be a clique of size smaller than $N = 5$. As seen in Figure~\ref{fig:clique3}, the clique finding algorithm returns a clique of size $4$ with values $\{29, 128, 209, 239 \}$ that results in database $\mydb{29, 99, 81, 30}$. Figure~\ref{fig:clique4} shows another clique of size $4$ with values $\{29, 209, 239, 299\}$ that results in database $\mydb{29, 180, 30, 60}$. It can be observed the two databases \emph{approximately} ``match'' in some locations, i.e. $\mydb{29, 180 (99 + 81), 30}$. It is important to note that although in this example $180$ is exactly equal to $99+81$, this need not hold in general, thus we consider two sequences a match if their corresponding values are \emph{approximately} equal. Having established this long match, we can deduce that value $60$ also belongs to the database and we can ``extend'' the initial candidate to include $60$ and return the database $\mydb{29, 99, 81, 30, 60}$. In another scenario assume we first detect the database of Figure~\ref{fig:clique4} and then we discover the database in Figure~\ref{fig:clique3}. In that case we can see that we can rewrite the initial candidate, i.e. $\mydb{29, 180, 30, 60}$ as $\mydb{29,180=(99+81),30,60}$ using the second candidate.


\begin{figure*}[h]
\centering
\begin{subfigure}[t]{0.20\textwidth}
\includegraphics[width=\textwidth]{figures/clique1.pdf}
\subcaption{The graph constructed from the \emph{exact} volumes of the database $[30, 100, 80, 30, 60]$ and the maximal clique corresponding to that.}
\label{fig:clique1}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.20\textwidth}
\includegraphics[width=\textwidth]{figures/clique2.pdf}
\subcaption{The graph constructed from the \emph{approximate/noisy} volumes of the database $[30, 100, 80, 30, 60]$. An edge in the maximal clique is missing.}
\label{fig:clique2}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.20\textwidth}
\includegraphics[width=\textwidth]{figures/clique3.pdf}
\caption{A maximal Clique in a graph with \emph{approximate/noisy} volumes.}
\label{fig:clique3}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.20\textwidth}
\includegraphics[width=\textwidth]{figures/clique4.pdf}
\caption{Another maximal Clique in a graph with \emph{approximate/noisy} volumes.}
\label{fig:clique4}
\end{subfigure}
\caption{The graph constructed from the \emph{exact} volumes has a maximal clique which can be used to recover the original database, while the noisy volumes might have smaller maximal cliques and the original database can not be recovered from just one clique.}
\label{fig:explain}
\end{figure*}

We next describe in detail the main steps taken in the Match \& Extend algorithm.
%in the case that the volumes are approximate/noisy and the noisy clique finding algorithm fails to find a clique of size $N$. 
The high level steps of the Match \& Extend can be found in Algorithm~\ref{alg:match_extend}.
We note that, in some cases,
simply increasing the noise budget allows us to  successfully find a clique of size $N$. However, as we will discuss in Section~\ref{sec:experiments}, by not increasing the noise budget and instead running the Match \& Extend algorithm, we can recover a database that is closer to the true database.
%We note that in some cases it may be advantageous to run the Match \& Extend algorithm, even when the noisy clique algorithm successfully finds a clique of size $N$,
%since the database reconstructed by using Explain will be closer to the true database. This will be discussed in further detail in Section~\ref{}.

\begin{algorithm}
\scriptsize
\SetAlgoLined
\KwResult{A database with $N$ values}
 \basesol\ = FindMaximalClique()\;
 allCliques = FindRemainingCliques(K, $\ell$)\;
%  i = 0\;
 \While{length(\basesol) < N}{
 \candsol = FindBestCandidate(allCliques)\;
 \basesol = Merge(\basesol, \candsol)
 }
 \Return \basesol
 \caption{Match \& Extend Algorithm}
 \label{alg:match_extend}
\end{algorithm}

%\vspace{-10mm}

\paragraph{FindMaximalClique} The first step in the Match \& Extend algorithm is to find a maximal clique in the constructed graph. Let $K$ denote the size of a maximal clique recovered in this step. If there is more than one clique with the same maximal size select one of them arbitrarily. Once the clique is found, the corresponding database is computed. We call this database \basesol\ and the rest of the algorithm will expand this database. If the size of maximal clique found in this step is $N$ we are done, otherwise the Match \& Extend algorithm expands the \basesol.

%\vspace{-3mm}

\paragraph{FindRemainingCliques} Recover all cliques of size ${K, K - 1, K - 2, \ldots, K - \ell}$ and sort them from the largest clique size to the smallest. For each clique, the corresponding database is found and is called \candsol. The \candsol\ is in the form of an ordered list of volumes that correspond to neighbouring ranges of the database. Note that the cliques to be found in this step are not restricted to be from the ranges in the form $\range{1}{1}, \range{1}{2}, ..., \range{1}{K}$ for some $K$. In fact, and this holds in the noiseless setting too, any set of volumes corresponding to ranges of the form $\range{i}{i_1}, \range{i}{i_2}, \dots, \range{i}{i_k}$ where $i\leq i_1 < i_2 < \dots < i_k$ will form a clique of size $k$, provided that all the differences of the volumes corresponding to these ranges are present in our data. This fact will enable our algorithm to discover the volumes of different parts of the true database and ``merge'' those parts to recover the original database.

%\vspace{-3mm}

\paragraph{ApproximateLCSubstring} This is a subroutine that is invoked as a part of \textbf{Merge} function. Given a \basesol\ and a \candsol\ in form of lists of volumes of neighboring ranges, it finds the longest common substring of these solutions, i.e. the longest contiguous list of volumes where both solutions agree. We call this substring the \comsubsol. To find it, we use a standard \emph{longest common substring} algorithm with a modification that the elements of the substring need to be only approximately equal (as defined in Section~\ref{sec:noisy_clique}) to the corresponding elements of \basesol\ and \candsol. At termination this will return the \comsubsol\, and the starting and ending indices of \comsubsol\ in the two given solutions.

%\vspace{-3mm}

\paragraph{Merge} Given the \basesol\ and a \candsol\ in the form of lists of volumes, attempt to combine the information in them into one larger solution. We refer to this as ``merging'' the two solutions. The \textbf{Merge} function first invokes \textbf{ApproximateLCSubstring} to find the approximate longest common substring of the two solutions. After the longest common substring of the two solutions and the locations of this substring in the two solutions are found, there can still be volumes where the \basesol\ and \candsol\ agree, which are not recognized by the \textbf{ApproximateLCSubstring}. 
For example, if the \basesol\ is $\mydb{\textbf{29}, 99, 81, 30}$ and \candsol\ is $\mydb{\textbf{29}, 180, 30, 60}$, the \comsubsol\ may be found as $\mydb{\textbf{29}}$, however one can see that the two solutions agree at $\mydb{99, 81}$ as well, only in the \candsol\ this information appears as the volume of one range $\mydb{180}$ which is the union of those two neighboring ranges in \basesol. 
The merging algorithm identifies such cases and extends the \comsubsol\ accordingly. The algorithm searches for occurrences where a volume $v_i$ next to the end of the \comsubsol\ in one of the solutions (say in \basesol) is approximately equal to the sum of volumes $u_j, u_{j+1}, \dots , u_{j+r}$ for $r \ge 0$ next to the same end of the \comsubsol\ in the other solution (say \candsol). In such a case, it extends the \comsubsol\ by appending to it $\mydb{u_j, u_{j+1}, \dots , u_{j+r}}$, and changing endpoints of the \comsubsol\ in \basesol\ and \candsol. 
So in the database given above, the algorithm will look at the neighbors of $\mydb{\textbf{29}}$ and discover that $180 \approx 99 + 81$, and extend the \comsubsol\ to $\mydb{\textbf{29}, \textbf{99}, \textbf{81}}$. Then, the algorithm will look at the neighbors of $\mydb{\textbf{29}, \textbf{99}, \textbf{81}}$ and discover that $30 \approx 30$, extending the \comsol\ further to $\mydb{\textbf{29}, \textbf{99}, \textbf{81}, \textbf{30}}$. It is important to mention that while the values in the example were exactly equal, the algorithm accepts values which are approximately equal as well, meaning that we look for whether $180 \stackrel{?}{\approx} 99 + 81$ or whether $30 \stackrel{?}{\approx} 30$. 
After the \comsubsol\ is maximally extended, our two solutions will have the following form: $\basesol\ = 
\mydb{\pref{1}, \comm, \suff{1}}$ and $\candsol\ = \mydb{\pref{2}, \comm, \suff{2}}$, where \comm\ is the \comsubsol\ found as previously explained, and any of the prefixes and suffixes may be empty. 
The algorithm then will do one of four things: (a) if \pref{1} (similarly, \suff{1}) is empty, it will extend the \comsubsol\ to $\comm\ = \pref{2} || \comm\ $ (similarly, $\comm\ || \suff{2}$), (b) if \pref{2} (similarly, \suff{2}) is empty, it will extend the \comsubsol\ to $\comm\ = \pref{1} || \comm\ $ (similarly, $\comm\ || \suff{1}$), (c) if both \pref{1} and \pref{2} (similarly, \suff{1} and \suff{2}) are of length 1, meaning they both contain one volume (say, $a$ and $b$, with $a<b$), and if the absolute value of the difference of these volumes appears in our volume measurements, then $\comm\ = \mydb{b-a, a} || \comm\ $ (similarly $\comm\ = \comm\ || \mydb{a, b-a})$, (d) if none of the above conditions are satisfied, the algorithm will abort the merge and repeat its steps for another \candsol. The condition (c) above is for identifying the cases where the volume in, say, \suff{1} corresponds to a range $\range{i}{j}$, which includes in itself the range of the volume in \suff{2}, which can be $\range{i}{k}$ for $k<j$. If the difference of these two volumes appears in the measured volumes, that difference likely corresponds to the range $\range{k+1}{j}$, so we replace $\mydb{b}$ ($\range{i}{j}$) by $\mydb{a,b-a}$ (which is the range $\range{i}{k}$ and range $\range{k+1}{j}$, respectively).

Back to our example database of $\mydb{30, 100, 80, 30, 60}$, we had last found the \comsubsol\ to be $\mydb{\textbf{29, 99, 81, 30}}$. In the merge step, we are going to have $\basesol = \mydb{ \comm }$ and $\candsol = \mydb{ \comm, 60}$. This falls under the case (a) where \suff{1} is empty, so the algorithm appends \suff{2} = $\mydb{60}$ to the \comsubsol\ and returns the solution as $\basesol = \mydb{\textbf{29, 99, 81, 30, 60}}$.
%\anote{in the last sentence it is still not clear to me why we have a,b-a and  not b-a, a for example} \mnote{tried to address above}

%\vspace{-3mm}

\paragraph{FindBestCandidate} Any time a merge is successful, two solutions are combined into one to create a larger solution. The reason why this larger solution was not initially found by the clique finder is that some volumes or connections in the graph were missing, and so a potential clique corresponding to this solution could not be formed. Every merge of two solutions identifies the number of missing volumes that prevented the combined solution from being found in the first place; in fact, if we were to add those missing volumes to the graph and start the algorithm again, the combined ``merged'' solution would show up among all listed solutions. Therefore we use the number of missing volumes as a metric for assessing the \emph{goodness} of a candidate solution; if there are few missing volumes, it suggests that the \basesol\ and \candsol\ agree in many volumes of the database, and are thus compatible, whereas if there are many missing volumes, the two solutions likely have different information about the volumes. The \textbf{FindBestCandidate} finds the candidate solution among all cliques that has the least number of such missing volumes with respect to being merged with the \basesol.

% The algorithm will check if \pref{1}\ and \pref{2}, and \suff{1}\ and \suff{2}\ describe the same volumes of the database, by referring to the graph and the reconstructed set of noisy volumes. Say, if \suff{1}\ is of the form $[\texttt{u + v}]$, and \suff{2}\ is of the form $[\texttt{u}]$, the algorithm will check if \texttt{v} appears among the noisy volumes (which would imply that the nodes corresponding to \texttt{u + v} and \texttt{u} are connected), and if so, it will extend $\comm = \comm\ ||\ [\texttt{u,v}]$, i.e. by appending the two new values $\texttt{u, v}$. 
% The algorithm will continue doing this on the remainder of \suff{1}\ and \suff{2}, until the end of both solutions is reached. In case if (only) one of the two \suff's is empty, the algorithm will extend \comm\ by appending to it the remainder of the other \suff. Using the rules described above, the algorithm will continually try to extend \comm\ from both endpoints, until a common solution that agrees with both initial solutions is formed. 

%\mnote{do we want to include an example with the steps of the merge algorithm here?}
%\mnote{not finished}.


%\paragraph{try to update the graph with the new volumes}\anote{add volume} After a merge has succeeded, the base solution has changed and increased in length. We find the volumes of all the ranges in this new base solution and add to our graph the ones that are missing. Then, we recompute the cliques and start over.\anote{we don't start over...}

\iffalse
\subsection{Error Reduction Step}\label{sec:CVP}

As explained in the previous section by using the noisy clique-finding and Match \& Extend algorithms on the noisy data we get some \textit{close} answer to the real database. Here we outline a technique which can reduce the noise and output a \textit{more accurate} answer. The first step is to compute all the $\binom{N}{2} + N$ volumes corresponding to each range. Specifically, the ranges $\range{1}{1}, \range{1}{2}, \ldots, \range{1}{N}$ are obtained using noisy clique-finding or Match \& Extend. %\mnote{Match \& Extend actually outputs [1-1], [2-2], ... [N-N]. I think we should change this here.}\anote{addressed} 
Each range $\range{i}{j}$ can be computed from the elementary volumes as $\size{\range{i}{j}} = \size{\range{1}{j}} - \size{\range{1}{i-1}}$. Instead of taking the computed value for range $\range{i}{j}$, we choose the value in the set of volumes (obtained from the side-channel data) that is closest to this computed value. This procedure results in $N' = \binom{N}{2} + N$ volumes which we call \emph{candidate volumes}.
Now note that given the volumes of the ranges $\range{1}{1}, \range{2}{2}, \ldots, \range{N}{N}$, the volume of any other range $\range{i}{j}$ can be expressed as a \emph{linear combination} of these values. Therefore, our variable $\vec{x} = (x_1, \ldots, x_N)$ corresponds to the volumes of the ranges $\range{1}{1}, \range{2}{2}, \ldots, \range{N}{N}$ and our candidate volumes $ \vec{v} = (v_1, \ldots, v_{N'})$, correspond to noisy linear combinations of the $x_i$'s. Thus, solving for the $\vec{x}$ which yields the closest solution to $ \vec{v} = (v_1, \ldots, v_{N'})$
under the linear constraints, corresponds to solving a Closest Vector Problem (CVP).

For example, if the range has size $N = 3$, then we obtain a total of $6$ volumes $v_1, \ldots, v_6$ corresponding to the ranges $\range{1}{1}$, $\range{2}{2}$, $\range{3}{3}$, $\range{1}{2}$, $\range{2}{3}$, $\range{1}{3}$ and can construct the following system of equations:
\[
\mathbf{A} \vec{x} + \vec{e} = \vec{v}
\]

where 
\[
\mathbf{A}=
\left[ {\begin{array}{ccc}
1 &0 &0\\
0 &1 &0\\
0 &0 &1\\
1 &1 &0\\
0 &1 &1\\
1 &1 &1
\end{array} } \right]
\]
$\vec{v} = (v_1, \ldots, v_6)$, $\vec{e}$ is the amount of error and $\vec{x}$ is unknown. To solve this problem, we can consider the lattice defined by $\mathbf{A}\vec{z}$, where $\mathbf{A}$ is the basis and $\vec{z}$ is any integer vector. Now, given $\vec{v}$, we would like to find the closest lattice vector $\vec{y} = \mathbf{A}\vec{x'}$ to $\vec{v}$. Once we have $\vec{y}$, we can solve to get $\vec{x'}$.

%\anote{maybe add a note saying why we are changing matrix A, telling the solver wants this}
To create a full rank matrix for our solver, we can modify matrix $A$ as following:
\[
A' =
\left[ {\begin{array}{cccccc}
1 &0 &0 &0 &0 &0\\
0 &1 &0 &0 &0 &0\\
0 &0 &1 &0 &0 &0\\
1 &1 &0 &T &0 &0\\
0 &1 &1 &0 &T &0\\
1 &1 &1 &0 &0 &T
\end{array} } \right]
\]
where $T \gg n$ and $\vec{v}$ stays the same.

Now we obtain a solution of dimension $6$ (as opposed to dimension $3$), but the last three coordinates should always be $0$, since if they are non-zero there will be at least $\pm$ $T$ in the corresponding coordinate of $\vec{v}$ \mnote{did we mean coordinate of $\vec{y}$?}\anote{it should be okay...}\mnote{can we review this part again? Maybe above we could say $\vec{v'}=\mathbf{A}\vec{x'}$, and here say "in the corresponding coordinate of $\vec{v'}$}, which will clearly not be the closest vector.

\fi

\iffalse

\subsection{(Enhanced?) Expectation Maximization}\anote{raw draft, I need to explain what is observation}
Expectation Maximization (EM) is an iterative process which will estimate the parameters of the distribution given the finite amount of observation. In this work the observation is the volume of the response to a particular query and the hidden variable is the query. Given that our measurement of the volume comes from the cache measurement and hence they are ineherently noisy, we use EM algorithm as the first step to find the best set of parameters which maximize our observation. The specific EM algorithm which we consider is Gaussian Mixture Model. From the observation we had from our measurement we made this assumption. 

Figure~\ref{fig:1vol} shows the result of running our attack on the scenario where only one range is being queried. As it can seen the correct volume stands out and the shape of the distribution is close to gaussian. The first step of our attack is to find the gaussians distribution which maximizes the likelihood of our observation.  


\begin{figure}
 \centering
  \includegraphics[width=0.7\linewidth]{figures/1vol.pdf}
  \caption{The volume of the response as a result of range query is . Since the cache measurement are noisy, we observe the noisy version of the volume.}
  \label{fig:1vol}
\end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{|c|ccc|}
\hline
\begin{tabular}[c]{@{}c@{}}Column\\ Distribution\end{tabular}              & \multicolumn{1}{c|}{Instance \#} & \multicolumn{1}{c|}{CorrectVolume} & Total Volume \\ \hline
\multirow{5}{*}{Uniform}    
    & 1 & 120/120 & 466 \\
    & 2 & 120/120 & 375 \\
    & 3 & 116/120 & 452 \\
    & 4 & 116/120 & 440 \\
    & 5 & 118/120 & 450 \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Narrow\\ Gaussian\end{tabular}} 
    & 1 & 118/120 & 474 \\
    & 2 & 110/120 & 492 \\
    & 3 & 114/120 & 493 \\
    & 4 & 112/120& 495 \\
    & 5 & 119/120 & 451 \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Wide\\ Gaussian\end{tabular}}   
    & 1 & 116/120 & 451 \\
    & 2 & 118/120 & 435 \\
    & 3 & 119/120 & 434 \\
    & 4 & 119/120 & 453 \\
    & 5 & 116/120 & 431 \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Real\\ Database\end{tabular}}   
    & 1 & & \\
    & 2 & & \\
    & 3 & & \\
    & 4 & & \\
    & 5 & & \\ \hline
\end{tabular}
\end{table}



\begin{figure}
 \centering
  \includegraphics[width=0.7\linewidth]{figures/em_res.pdf}
  \caption{TBD}
  \label{fig:em_res}
\end{figure}

 
\subsection{NLS}
Once the potential volumes are recovered 




\subsection{Applying Subgraph Isomorphism Solver--Noiseless Case}\label{sec:subgraph_iso_noiseless}

We describe a procedure
for finding candidate solutions for the reconstructed database by using a subgraph isomorphism solver. 
We first describe the procedure for \emph{noiseless} data,
where we are given the exact values of all
$\binom{N}{2} + N$ number of volumes.
In the next section, we describe how to extend to the noisy case.

%As we will see, the candidates obtained by the procedure are fairly noisy. Specifically, the volume which is recovered by the previous procedure might be $1$ or $2$ off. \dnote{would be good to have some quantitative numbers here}\anote{tried to add something to give a sense} We will therefore apply the techniques in the following section to further reduce the noisy.

Recall that in the subgraph isomorphism problem, we must construct a ``pattern graph'' $H$, and a ``target graph'' $G$. The solver will then find the isomorphic copies of $H$ contained in $G$.
We construct the pattern graph $H$ using only the structure of the range queries, in a way that is independent of the database itself. Then we proceed to construct the target graph $G$ from the empirical measurements obtained from the cache. Next we call the subgraph isomorphism on pattern graph $H$ and target graph $G$. The subgraph isomorphism gives the mapping from pattern graph $H$ to target graph $G$. Since the pattern graph represent the ranges and target graph represent volumes, it means that subgraph isomorphism solver assigns a value to each range. All solutions output by the subgraph isomorphism solver are candidates for the (volumes of all range queries within the) reconstructed database. In the following we describe each part of the reconstruction attack in detail.

\dnote{Include figure depicting the pattern graph.}\anote{ Figure \ref{fig:pattern_graph}}

\paragraph{Constructing The Pattern Graph}\label{sec:pattern_graph_noiseless}
In order to build the pattern graph $H$ we construct a \emph{directed} graph where each node in the graph corresponds to a different range query. Assuming the range of values are from $1$ to $N$ there are $\binom{N}{2} + N = \frac{N(N+1)}{2}$ possible ranges, and therefore $\frac{N(N+1)}{2}$ number of nodes in the graph. Each range $[i-j]$ is represented by a node. For each node $[i-j]$ we include an edge to node $[i'-j]$ for $i < i' \leq j$. Similarly we include an edge to node $[i-j']$ for $i \leq j' < j$. Figure~\ref{fig:pattern_graph} shows an example of portion of pattern graph. In this example we focus on the connections going out from node $[1-4]$. It is connected to $3$ nodes which are of the form $[i'-j]$, namely $[2-4],[3-4],[4-4]$. It is also connected to $3$ nodes which are of the form $[i-j']$, namely $[1-1],[1-2],[1-3]$. Node $[1-4]$ has some incoming edges as well and the rest of the nodes have some other outgoing edges as well. It is worth mentioning that nodes of the form $[i-i]$ has no outgoing edges and these are the nodes representing the volumes which we are interested in. 
\anote{figure and explanation added}

\begin{figure}
 \centering
  \includegraphics[width=\linewidth]{figures/pattern_graph.pdf}
  \caption{Pattern graph showing all the outgoing connections of the node $[1-4]$. A node in the form $[i-j]$ ($[1-4]$ in this Figure) is connected to nodes in the form $[i'-j]$ (left half) with $i < i' \leq j$ and nodes in the form $[i-j']$ (right half) with $i \leq j' < j$. In this figure nodes in the form $[i'-j]$ are $[2-4],[3-4],[4-4]$ and nodes in the form $[i-j']$ are $[1-1],[1-2],[1-3]$.}
  \label{fig:pattern_graph}
\end{figure}

\dnote{Describe how the target graph is constructed from the data}
\dnote{It might be easier to first discuss how the target graph is constructed, given \emph{perfectly} correct data. Then add a paragraph explaining how the target graph is constructed from the actual empirical
data.}\anote{done}

\paragraph{Constructing The Target Graph from Exact Volumes}\label{sec:target_graph_noiseless}
Given a multi-set $\mathsf{S}$ of $\binom{N}{2} + N$ number
of exact volumes, we construct the target graph in the following way:
Each volume $v \in \mathsf{S}$ is corresponds to a node in the graph. We include an edge from node $a$ to node $b$ if there is a volume $c \in \mathsf{S}$ such that $a = b + c$. The reason is that if this equation holds, then the nodes $(a, b, c)$ might correspond to the ranges $a \leftrightarrow [i-j]$, $b \leftrightarrow [i- j']$, $c \leftrightarrow [(j'+1)- j]$ for some $i \leq j' < j$. If $(a,b,c)$ do not satisfy this equation,
then we know that $(a,b,c)$ cannot correspond to ranges of this form.

\dnote{Explain why an isomorphic subgraph solves the problem. I.e. if we find an isomorphic subgraph then what do we take as the solution to the database reconstruction problem and why.}
\paragraph{Reconstruction--Noiseless Case}
By now we have pattern and target graph constructed as mentioned. The edges in the pattern graph are from node $[i-j]$ to nodes $[i'-j]$ and $[i-j']$. Note that these edges also presents in the target graph, due to the way we constructed it: Recall, the way to construct the target graph was to connect node $a$ to node $b$ if there exists another node $c$ satisfying $a = b + c$. In the pattern graph node $a$ is $[i-j]$, node $b$ is $[i'-j]$ (or $[i-j']$) and node $c$ is $[i-(i'-1)]$ (or $[(j'+1)-j]$). So  connections which are in the pattern graph are also present in the target graph. Once the subgraph isomorphism is called on the two graphs the answers are in the form where it assigns each node from the pattern graph (in the form $[i-j]$) to a value from the target graph (in the form $a$). As mentioned, in total there are $\frac{N \big(N+1\big)}{2}$ ranges and for each we obtain a mapping to its volume. Among all these ranges there are ranges in the form of $[1-1],[2-2], \ldots, [N-N]$. These are exactly the database entries we were looking for and therefore using the subgraph isomorphism solution we may return those as an answer to database reconstruction. 



\begin{figure}
 \centering
  \includegraphics[width=0.6\linewidth]{figures/full_pattern_graph2.pdf}
  \caption{Complete pattern graph constructed for the case where $N = 3$. For example there is connection from range $[1-2]$ to range $[1-1]$ and range $[2-2]$ as they are in the format specified in Section~\ref{sec:pattern_graph_noiseless}.}
  \label{fig:full_pattern_graph}
\end{figure}

\dnote{I'm not sure Figure~\ref{fig:full_pattern_graph} is depicting 
what we want. We want to show that the target graph has more edges than
the pattern graph and that the subgraph isomorphism solver essentially tells us which edges are the ``extraneous'' edges. Maybe to show this, you can give an example where $v_1, \ldots, v_6$ are set to some real values and show how the underlying graph is present, but also some extraneous edges that do not ``belong.''}

\paragraph{End to End Example--Noiseless Case}
As an example lets look at Figure~\ref{fig:full_pattern_graph} and Figure~\ref{fig:full_target_graph}, which shows a pattern graph and target graph, respectively. Figure~\ref{fig:full_pattern_graph} is constructed solely by knowing the possible ranges. For example we include an edge from $[1-2]$ to $[1-1]$ and $[2-2]$ since they are in the format specified in Section~\ref{sec:pattern_graph_noiseless}. For the target graph we assume the original database was $\{5,11,10\}$. Assume we get volumes $\{5,10,11,16,21,26\}$. We construct them solely by the rule specified in Section~\ref{sec:target_graph_noiseless}. As it can be seen in Figure~\ref{fig:full_target_graph} there is a connection from node $21$ to $5$ since there exists another node i.e. $16$ such that $21 = 5 + 16$. As it can be seen in Figure~\ref{fig:full_target_graph} the target graph has potentially more edges than pattern graph. Given two graphs in Figure~\ref{fig:full_pattern_graph} and Figure~\ref{fig:full_target_graph} to subgraph isomorphism solver it will assign each ranges of pattern graph a value which is also shown in Figure~\ref{fig:full_target_graph}. Although we are only interested in ranges $[1-1] = 5, [2-2] = 11, [3-3] = 10$ the subgraph isomorphism outputs potential value for other ranges as well i.e. $[1-2] = 16, [2-3] = 21, [1-3] = 26$. Finally the original database is reconstructed this way.  

\begin{figure}
 \centering
  \includegraphics[width=0.6\linewidth]{figures/full_target_graph2.pdf}
  \caption{Construction of Target graph for noiseless case. Assume the observed volumes are $\{5,10,11,16,21,26\}$. There is a connection from node 21 to 5 since the exist another node i.e. 16 such that 21 = 5 + 16. The construction of target graph is explained in Section~\ref{sec:target_graph_noiseless}.}
  \label{fig:full_target_graph}
\end{figure}

\subsection{Applying Subgraph Isomorphism Solver--Noisy Case}\label{sec:subgraph_iso_noisy}

In this case, the pattern graph is constructed in the same
way as described above. However, constructing the target graph
is performed differently, as described next.

\paragraph{Constructing The Target Graph from Empirical Data}\label{sec:target_graph_noisy}
\dnote{Please update this section. I'm not sure
it's describing what we actually do. Don't we duplicate the volumes and then require exact equivalence in the target graph.}

The target graph $G$ is built from the timing data obtained from cache activity. As explained in Section~\ref{sec:aprox_vol} the cache is monitored during each range query execution. The experiments are repeated until \textit{good} confidence in the number value of the volume is obtained. Experimentally for the case of $N=10$ we conducted the experiment for $30,000$ time and gathered the traces for them. After performing some signal processing we get the approximate value for volumes. As it can seen in Figure~\ref{fig:volume_attack} each volume which occurred a number of times higher than a certain threshold (set empirically) will be accepted as a potential volume and we will construct the target graph based on that. The obtained volumes are duplicated since there might be two ranges which gives equal volumes. Each volume will be treated as a node and we include an edge from node $a$ to node $b$ if there is another volume $c$ such that $| b + c -a | = 0$. The reason behind why the target graph is constructed in this way is explained in Section~\ref{sec:target_graph_noiseless}. The measurement from cache have correct volumes among other noisy volumes which introduced during our measurements from cache. So the difference between the noiseless case and noisy one is addition of extra volumes as well as extra edges.  
%The reasoning behind this equation is that if all our data was perfect and we could reconstruct the perfect value for each volume we could modify the edge connection criteria such that $b + c = a$ but since the cache measurements are noisy we modify the criteria to be able to tolerate noise. The noise we observed in our measurement makes the value of each volume to be wrong by $\pm 1$ so by setting a adding an edge in cases where there are off by $2$ we tolerate for that noise. 
\dnote{The last sentence is pretty unclear.}
\anote{added description}

\paragraph{Reconstruction--Noisy Case}
In the case of noisy data, there are potentially more nodes, as well as edges, in the target graph compared to the pattern graph. This is not problematic for the subgraph isomorphism solver as it will simply look for a subgraph in the target graph and will output a solution which satisfies isomorphism from pattern graph to target graph. Similar to noiseless scenario, the solution in this case has $\frac{N(N+1)}{2}$ potential answers for the nodes in the pattern graph. In this case we use this potential answer as a solution which is \textit{close} to the actual solution and we will use the procedure explained in the next section namely \textbf{CVP Solver} to get even \textit{closer} answers to the real solution.
\anote{added this section}
Indeed, we have observed experimentally that the subgraph isomorphism solver is robust and can be applied in the noisy
setting to obtain fairly good approximate reconstructions.
We discuss our experimental results further in Secion~\ref{sec:experiments}.
As we will see, the candidates obtained by the procedure remain fairly noisy. 
%Specifically, the volume which is recovered by the previous procedure might be $1$ or $2$ off. \dnote{would be good to have some quantitative numbers here}\anote{tried to add something to give a sense} 
We will therefore apply the techniques in the following section to further reduce the noise.
\dnote{The following requires another pass.}
\dnote{Is this even relevant any more? We don't construct the target graph in this way. Don't we now duplicate the volumes and then require exact 
equivalences? So the assumption in the theorem should be something like if after duplicating all the empirical volumes, we are guaranteed to contain all the true volumes (including multiple instances of the same volume).}

\iffalse
\begin{theorem}
Let $D$ be a correct database.
Consider a multiset $\mathsf{S}$ that consists of $N' \geq {N \choose 2} + N$ noisy volumes, each corresponding to noisy measurements for a range $[i,j]$. Assume furthermore that each noisy volume is within $\pm 1$ of the correct volume in database $D$.
Consider the pattern graph $H$ described above
and the target graph $G_\mathsf{S}$ constructed from
$\mathsf{S}$.
Then there exists a subgraph $G'$ in $G_\mathsf{S}$ isomorphic to $H$.
\end{theorem}

\begin{proof}
We first define a subgraph $G''$ of $G_\mathsf{S}$.
We then argue that $H$ is isomorphic to a subgraph of $G''$.

\noindent
\textbf{Subgraph $G''$.}
Recall that we assume that multiset $\mathsf{S}$ consists of $N' \geq {N \choose 2} + N$ noisy volumes, each corresponding to noisy measurements for a range $[i,j]$. Furthermore we assume that each noisy volume is within $\pm 1$ of the correct volume in database $D$.
Let each entry in $D$ be denoted by an ordered pair
$([i-j], v)$, where $[i-j]$ is the range and $v$
is the volume.
Then there must exist a mapping $\pi$ that maps ranges $[i-j]$ to volumes $v' \in \mathsf{S}$
such that
$\pi([i-j]) = v'$ implies that $([i-j], v) \in D$
and $v' \in v \pm 1$.
Let the subgraph $G''$ consist of the volumes
$v'$ that are mapped to some range $[i-j]$ by $\pi$,
as well as all edges in $G_\mathsf{S}$ among those nodes.

We have now constructed a graph $G''$ and a mapping $\pi$ from nodes in $H$ to nodes in $G''$.
We now show for every edge in $H$ from $[i-j]$ to $[i'-j']$,
there exists an edge in $G$ from 
$\pi([i-j])$ to $\pi([i'-j'])$.
Assume there is in edge in $H$ from $[i,j]$ to $[i'-j']$.
This means that $[i'-j'] \subsetneq [i-j]$
and either $i' = i$ or $j' = j$.
Therefore in $D$, there must exist 
pairs
$([i-j], v_1)$, $([i'-j'], v_2)$, $([i''-j''], v_3)$
such that
$v_1 = v_2 + v_3$.
Then $\pi([i-j])$ (reps.~$\pi[i'-j'], \pi[i''-j'']$) corresponds to a node
$v'_1$ (resp.~$v'_2, v'_3$) of volume $v'_1 \in v_1 \pm 1$ (reps. $v'_2 \in v_2 \pm 1, v'_3 \in v_3 \pm 1$)
in $G''$.
Therefore,
$v'_2 + v'_3 -3 \leq v'_1 \leq v'_2 + v'_3 + 3$.
Thus, the corresponding edge exists in $G''$,
by the definition of construction of $G_{\mathsf{S}}$.
\end{proof}
\fi

\subsection{Applying CVP Solver} \label{sec:CVP}
As explained in the previous section by using the subgraph isomorphism on the noisy data we get some \textit{close} answer to the real database. Here we explain a technique which can remove the noise and output a \textit{more accurate} answer.

We transform the problem of extracting the correct database, given $\binom{N}{2} + N$ number of noisy volumes, corresponding to each of the $\binom{N}{2} + N$ number of ranges.
Specifically, given the volumes of the ranges 
$[1-1], [2-2], \ldots, [N-N]$, we note that every other range
$[i-j]$ can be expressed as a \emph{linear combination} of these values.
Therefore, our variable $x$ corresponds to the volumes of the 
ranges $[1-1], [2-2], \ldots, [N-N]$ and our
candidate volumes $(v_1, \ldots, v_{\binom{N}{2} + N})$,
output by the subgraph isomorphism solver,
correspond to noisy linear combinations of $x$.
Thus, solving for $x$ which yields the closest
solution to $(v_1, \ldots, v_{\binom{N}{2} + N})$
corresponds to solving a Closest Vector Problem (CVP).

\dnote{Give a small end-to-end example like from my emails.}

For example, if the range has size $N = 3$, then we obtain a total of $6$ volumes $v_1, \ldots, v_6$ corresponding to the ranges $[1-1]$, $[2-2]$, $[3-3]$, $[1-2]$, $[2-3]$, $[1-3]$ and can construct the following system of equations:
\[
A \vec{x} + \vec{e} = \vec{v}
\]

where 
\[
A=
\left[ {\begin{array}{ccc}
1 &0 &0\\
0 &1 &0\\
0 &0 &1\\
1 &1 &0\\
0 &1 &1\\
1 &1 &1
\end{array} } \right]
\]
$\vec{v} = v_1, \ldots, v_6$,
$\vec{e} \in [\pm 2]^6$
and $\vec{x}$ is unknown.

To solve this problem, we can consider the lattice defined by $A\vec{x}$, where $A$ is the basis and $\vec{x}$ is any integer vector. Now, given $\vec{v}$, we would like to find the closest lattice vector $\vec{y} = A\vec{x'}$ to $\vec{v}$. Once we have $\vec{y}$, we can solve to get $\vec{x'}$.

\anote{maybe add a note saying why we are changing matrix A, telling the solver wants this}
We can modify matrix $A$ as following:
\[
A' =
\left[ {\begin{array}{cccccc}
1 &0 &0 &0 &0 &0\\
0 &1 &0 &0 &0 &0\\
0 &0 &1 &0 &0 &0\\
1 &1 &0 &T &0 &0\\
0 &1 &1 &0 &T &0\\
1 &1 &1 &0 &0 &T
\end{array} } \right]
\]
where $T \gg n$ and $\vec{v}$ stays the same.

Now we obtain a solution of dimension $6$ (as opposed to dimension $3$), but the last three coordinates should always be $0$, since if they are non-zero it will add at least $\pm$ $T$ to the corresponding coordinate of $v$, which will clearly not be the closest vector.

\subsection{Incorporating Auxiliary Information about Query Distribution}\label{sec:aux_query}
\dnote{Aria--please describe your attack that decides which volumes to duplicate or not duplicate based
on the knowledge that queries are uniformly random.}

As it was explained in the previous section, in order to construct the target graph \emph{all} the potential volumes will be duplicated. In this section we explain how by assuming that the distribution of the queries are uniform we can only add volumes which are more likely to be repeated. As it can seen in Figure~\ref{fig:volume_attack} there are some volumes which occur significantly more than their neighbouring volumes. Assuming the query distribution is uniformly random, that means that the volumes which occurs more frequently correspond to the volumes which are coming from two different ranges. Those are the volumes which are candidate to be duplicated. Since cache measurements are affected by the noise of the system, the queries on the bigger ranges (hence bigger volumes) are more noisy that smaller ranges. So there is a less chance of having perfect traces for bigger volumes. Hence we divide the whole ranges into smaller segments and in each segment we detect the volumes which happens more frequent than the rest and announce them as candidates for duplication.\anote{above needs another pass}


\subsection{Incorporating Auxiliary Information about the Data Distribution} \label{sec:aux_data}
In this section, we explain how we can 
incorporate
auxiliary information about the distribution of the data into the subgraph isomorphism problem instance. We focus on the case where each row is an i.i.d. variable drawn from a Gaussian distribution $D_{c, \sigma}$ of known mean $c$ and standard deviation $\sigma$.
In some cases, information about the distribution of a certain column can be obtained from public, auxiliary information. For example, United States Census Bureau releases income information for a certain Zip Code~\cite{USACensus}, we want to find out how many people in a certain income range.
\dnote{Aria--please give an example of why it is realistic. E.g. if distribution of SAT test scores are published and we want to find out how many students from a certain public high school had SAT test scores falling into each range of 100 points out of 1600.}
Given the known distribution $D_{c, \sigma}$, the \emph{expected value of each range} $[i,j]$ can be obtained. We will construct a subgraph isomorphism instance that enforces a mapping in which each range $[i,j]$ maps to an empirical volume that is within $\alpha \cdot \sigma$ (i.e.~$\alpha$ number of standard deviations) from its mean. Statistically, it would be very unlikely for any empirical volume to deviate by more than this from its mean. Towards this goal, we introduce additional nodes in both our pattern and target graphs which we called \emph{buckets}. Let $B$ bet the number of buckets added to to the pattern and target graphs, where each bucket corresponds to a range of volumes. For example, the first bucket corresponds to the range of volumes between $1$ and $n/B$, where $n$ is the size of the database; the $\ell$-th bucket corresponds to the range of volumes between $(\ell-1)\cdot n/B + 1$ and $\ell \cdot n/B$. In the pattern graph, we include an edge from range $[i,j]$ to bucket $\ell$ if the expected size of
range $[i,j]$ is between $(\ell-1)\cdot n/B + 1$ and $\ell \cdot n/B$ (See Figure~\ref{fig:bucket_pattern}). For example in Figure~\ref{fig:bucket_pattern}, both ranges $1-1$ and $1-2$ are mapped to bucket $1$, which means that the expected value of the volume for those two ranges is between $1$ and $n/B$. Additionally, each bucket has a special cycle structure (i.e.~a cycle graph of a particular size) attached to it. The cycle structure of bucket 1 is different than bucket 2. Specifically, the $\ell$-th bucket is associated with a cycle of size $\ell + 1$. 
\dnote{Is the above correct?}\anote{I will change it to $\ell + 1$ because that is what it is in the figure, in the experiments I used $\ell + 2$}
This cycle structure enforces that the $\ell$-th bucket in the pattern graph gets mapped to the $\ell$-th bucket in the target graph in each subgraph isomorphism that is found\footnote{Note that no cycles other than these exist in the pattern or target graphs, so they must be mapped to each other.}. For the target graph, for each node corresponding to volume $v$ (where $v$ represents a volume included from the empirical data), we include an edge to the $\ell$-th bucket if 
$(v + \alpha \cdot \sigma)$ or 
$(v - \alpha \cdot \sigma)$ fall within the range
$(\ell-1)\cdot n/B + 1$ and $\ell \cdot n/B$.
See Figure~\ref{fig:bucket_target}. As the values might deviate from their expected values, we chose the margin of error called $f = \alpha \cdot \sigma$. For example, for volume $v_1$, adding and subtracting the margin $f$, both $v_1 + f$ and $v_1 - f$ fall in bucket 1 (meaning that both of the values fell within the range between $1$ and $n/B$). It worth noticing that nodes corresponding to volumes $v$ can potentially get mapped to more than one bucket (e.g. $v_2$ in Figure~\ref{fig:bucket_target}). As in the pattern graph, there is a unique cycle structure attached to each bucket. As mentioned previously, this structure will enforce that the $\ell$-th bucket in the pattern graph gets mapped to the $\ell$-th bucket in the target graph. 

\begin{figure}
 \centering
  \includegraphics[width=0.6\linewidth]{figures/buckets_pattern.pdf}
  \caption{Enforcing expected value of each range in Pattern Graph. New nodes called bucket nodes are added to the graph which represent the range of volume. For each range $[i-j]$ we compute the expected value of it's volume and we connect it to the correct bucket. Extra cycles nodes are added to bucket node to guarantee the correct mapping from bucket in pattern graph to corresponding buckets in target graph.}
  \label{fig:bucket_pattern}
\end{figure}

\begin{figure}
 \centering
  \includegraphics[width=0.6\linewidth]{figures/buckets_target.pdf}
  \caption{Enforcing expected value of each range in Target Graph. New nodes called bucket nodes are added to the graph which represent the range of volume. For each volume $v_i$ add edges to bucket corresponding to values $v_i \pm f$ ($f$ being a value which volume might deviate from it's current value). Extra cycles nodes are added to bucket node to guarantee the correct mapping from bucket in pattern graph to corresponding buckets in target graph.}
  \label{fig:bucket_target}
\end{figure}

\subsection{Scaling to Large Databases and Ranges} \label{sec:efficient}
\dnote{Let's keep this section, and just suggest solutions that can
be investigated in future work.}
Complexity of subgraph isomorphism and CVP depend only on
the size of the range and not on the size of the database.
\dnote{Discuss how we can improve the complexity of CVP to be independent of the
size of the range by partitioning the problem into several instances of CVP, each for ranges of different lengths.}
However, the issue with dealing with large databases
is that the accuracy of the volumes we are able to recover
degrade as the database size grows.
Recall that
we detect the approximate value of each volume by tracking cache activity. As the size of the volume grows we must monitor a line for a longer period of time. This monitoring is noisy and as the volume increases there is a larger chance that significant noise will be introduced in our measurement due to operating system interrupt. Empirically, we found that volumes of size more than $1000$ can not be detected reliably. \dnote{e.g.~due to an operating system interrupt, which will cause some external code to run, thus polluting the cache (is this right?)}.
\dnote{Should add some experimental data on how large of a database we can handle before the noise gets too large.}

\fi



==> Database Cache Attack/background.tex <==
%\vspace{-3mm}
\section{Background} \label{sec:backgrounds}

% : the knowledge required to understand our attack/implications


%In this section, we describe a background of cache side-channels, followed by the knowledge needed to successfully mount a cache attack.

%\subsection{Cache Architecture}

%\vspace{-3mm}

\paragraph{Cache Architecture}
In order to reduce the access time to main memory, modern CPUs are equipped with multiple levels of cache. They form a hierarchy such that the Level 1 cache is the fastest and smallest, whereas the Level 3 cache is the slowest and largest. 

The Level 1 cache is divided into two separate caches, one holds the data and the other holds the instructions. In the higher level caches data and instructions are held in the same cache. Level 3 is a shared-memory space and is the Last Level Cache (LLC). The LLC is all-inclusive of the lower levels of the architecture, meaning that any data present in L1 and L2 is also present in the LLC.

Each cache comprises multiple sets and each set contains multiple cache lines. Each line of main memory is mapped to a unique cache set. Within this set, however, a memory line can be mapped to any of the cache lines. Typically, each line of cache holds 64 Bytes of data. Upon writing a line to a set that is already full, 
%\dnote{I think you mean ``set'' here?}\anote{Well I meant line I think it is more generic, because we technically write to a line and not a set}
a decision regarding which memory line to evict must be made. This decision is called a \emph{Replacement Policy} and depends on the cache architecture. A popular replacement policy is \emph{least-recently used (LRU)}, which replaces the least recently used entry with the new one. 

%\vspace{-3mm}

%\subsection{Flush+Reload Attack}
\paragraph{Flush+Reload Attack}
Caches are vulnerable to information leakage since an adversary who is co-located with the victim on the same processor can retrieve useful information about a victim's activities.
%The adversary can retrieve victim's activities through timing attacks. 
Specifically, the adversary can monitor its own access time to the cache and use deviations in access time to deduce information about whether or not the victim has accessed a certain memory line or not. The reason that such an attack is feasible is that the adversary and victim share the same resource i.e.~the cache. 
%on a physical machine through timing attacks on the last level cache. 
Moreover, in a setting where the adversary and victim share a library, they will both have access to the physical memory locations in which the \emph{single copy} of the library is stored. The attacker can now explicitly remove a line corresponding to the shared physical memory from the cache. To exploit the shared physical memory in a useful way, Yarom and Falkner introduced an attack called \emph{Flush+Reload}~\cite{184415}.
The attacker flushes a monitored line from the cache using a special command called \texttt{clflush}. This command causes the monitored line to be removed from the L1, L2 and L3 caches. As mentioned before, L3 is inclusive and as a result the removed line will be removed from all the other caches, even if the attacker and the victim are not on the same physical core.
The attacker then lets the victim continue to run its program. After some time has elapsed, the attacker regains control and measures memory access time to determine whether or not the monitored line is present in the cache.
If the monitored line is present in the cache (reloading runs fast), the attacker deduces that the same line was accessed by the victim during its run. If the monitored line is not present in the cache (reloading runs slow), the attacker deduces that the victim did not access the line during its run. 
Hence the attacker knows whether the victim accessed a specific line or not. 
In order to perform the Flush+Reload attack we used the package provided in the Mastik framework. Mastik~\cite{yarom2016mastik} is a toolkit with various implementations of published micro-architectural side-channel attacks. It provides an interface that can be used to set the monitored lines. For our work we used \texttt{fr-trace} to monitor various cache lines. 

%Another technique that, in general, helps the performance of cache attack is called a performance degradation attack~\cite{allan2016amplifying}. This technique targets specific lines in the program and by constantly flushing those lines makes the target program run slower. 
%This technique causes the target program to run slower and helps the attacker to have better timing resolution and catch more victim's activities.
%\dnote{Add a sentence here about \emph{why} it is beneficial for the attack to slow down the victim.}\anote{added}
%We used the \texttt{fr-pda} and target the most commonly executed lines.

%\vspace{-3mm}

%\subsection{Cache Prefetching}
\paragraph{Cache Prefetching}
When an instruction or data is needed from memory, it is fetched and brought into the cache. To reduce execution time further, \emph{Cache Prefetching} is implemented to bring a memory line into the cache \emph{before} it is needed. The prefetching algorithm decides what and when to bring data and instruction to the cache. Hence, when the program needs the data or instruction in the future, it will be loaded from the cache instead of memory. This is based on the past access patterns or on the compiler's knowledge.
%\dnote{Say something about how it decides which locations to pre-fetch?}\anote{done}
%Cache prefetching can either fetch data or instruction. 


\paragraph{Range Queries}
A range query is an operation on a database 
in which records with column values between a certain lower and higher bound are returned. Assuming there exists a column $c$ in a database with values between $1$ and $N$, the command $\texttt{range}[a,b]$ for $1 \leq a \leq b \leq N$ returns all the entries in the database which have a value in column $c$ in the range $[a,b]$ (inclusive for both $a$ and $b$).


\paragraph{Clique Finding Problem}
The Clique problem is the problem of finding a clique--a set of fully connected nodes--in a graph. 
We utilize the clique finding algorithm in the NetworkX Package.\footnote{NetworkX is a Python library for studying graphs and networks.} The NetworkX package can be used to find the clique number (size of the largest clique in the graph) as well as all cliques of different sizes in the graph.

%\subsection{Range Queries}
\iffalse
\paragraph{Range Queries}
A range query is an operation on a database 
in which records with column values between a certain lower and higher bound are returned. Assuming there exists a column $c$ in a database with values between $1$ and $N$. The command $\texttt{range}[a,b]$ for $1 \leq a \leq b \leq N$ returns all the entries in the database which have a value in column $c$ in the range $[a,b]$ (inclusive for both $a$ and $b$).

%\vspace{-3mm}

%\subsection{Clique Finding Problem}
\paragraph{Clique Finding Problem}
The Clique problem is the problem of finding a clique--a set of fully connected nodes--in a graph. 
%A set of nodes is called a clique if any two nodes in the set are connected by an edge.
%\dnote{Need to explain what is a clique?}\anote{done}
%The clique finding problem has usage in bioinformatics and in computational chemistry, among others.
We utilize the clique finding algorithm in the NetworkX Package\footnote{NetworkX is a Python library for studying graphs and networks.}. The NetworkX package can be used to find the clique number (size of the largest clique in the graph) as well as all cliques of different sizes in the graph. 
\fi
%\vspace{-3mm}

%\subsection{Closest Vector Problem (CVP)}
\iffalse
\paragraph{Closest Vector Problem (CVP)}
Given $n$-linearly independent vectors $\mathbf{b}_1, \mathbf{b}_2, \ldots, \mathbf{b}_n \in \mathbb{R}^m$, the lattice generated by $\mathbf{b}_1, \mathbf{b}_2, \ldots \mathbf{b}_n$ is the set of all the integer linear combination of them i.e. $\mathcal{L}(\mathbf{b}_1, \mathbf{b}_2, \ldots \mathbf{b}_n) = \{ \sum_{1}^{n}\mathbf{b}_i x_i\ | \ x_i \in \mathbb{Z}\}$. The set $\{ \mathbf{b}_1, \mathbf{b}_2, \ldots \mathbf{b}_n \}$ is called the basis of the lattice and is presented by matrix $\mathbf{B}$ in which basis $\mathbf{b}_i$ is $i$-th row of the matrix. In the closest vector problem target vector $\mathbf{y}$ is given. 
The target vector $\mathbf{y}$ does not necessarily belong to lattice $\mathcal{L}$. 
The solution is a lattice point $\mathbf{y}' = \mathbf{x}\mathbf{B}$ which is closest to target vector $\mathbf{y}$ and also $\mathbf{y}' \in \mathcal{L}$. Notice that a lattice point $\mathbf{y}'$ is a linear combination of basis, while the target vector $\mathbf{y}$ is not. The significance of the CVP problem is to find a closest vector to $\mathbf{y}$ such that the linear combination is satisfied.  CVP problem is also known to be NP-complete and we use \texttt{fplll}~\cite{fplll} for finding the closest vector in lattice.
\fi

\iffalse
\subsection{Closest Vector Problem (CVP)}

Given $n$-linearly independent vectors $\mathbf{b}_1, \mathbf{b}_2, \ldots, \mathbf{b}_n \in \mathbb{R}^m$, the lattice generated by $\mathbf{b}_1, \mathbf{b}_2, \ldots \mathbf{b}_n$ is the set of all the integer linear combination of them i.e. $\mathcal{L}(\mathbf{b}_1, \mathbf{b}_2, \ldots \mathbf{b}_n) = \{ \sum_{1}^{n}\mathbf{b}_ix_i\ |\ x_i \in \mathbb{Z}\}$. The set $\{\mathbf{b}_1, \mathbf{b}_2, \ldots \mathbf{b}_n\}$ is called the basis of the lattice and is presented by matrix $B$ in which basis $\mathbf{b}_i$ is $i$-th row of the matrix. In the closest vector problem target vector $\mathbf{y}$ is given. The solution is a lattice point $\mathbf{x}\mathbf{B}$ which is closest to target vector $\mathbf{y}$. CVP problem is also known to be NP-complete. We use \texttt{fplll}~\cite{fplll} for finding the closest vector in lattice. 


\subsection{Subgraph Isomorphism Problem}

The subgraph isomorphism problem is a computational task in which two graphs $G$ and $H$ are given. One must find a subgraph of $G$ such that it is isomorphic to graph $H$. Graph $H$ is called the pattern graph and graph $G$ is called the target graph. While the subgraph isomorphism is NP-complete, it is an important problem in various fields such as Chemistry or in general cases where people are interested in pattern matching.
%\dnote{put in something here--e.g. chemistry?}\anote{added}. 
Therefore, there has been significant effort in designing and implementing heuristic solvers that perform well in practice. 
In this project, we use \texttt{directedLAD} solver program which is Version 2 of the implementation provided in~\cite{subgraph_solver}.
%\dnote{put in the name of the solver}\anote{added}
\fi

==> Database Cache Attack/backup.tex <==

\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. Please do not use it for A4 paper since the margin requirements for A4 papers may be different from Letter paper size.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as Ò3.5-inch disk driveÓ.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ÒWb/m2Ó or Òwebers per square meterÓ, not Òwebers/m2Ó.  Spell out units when they appear in text: Ò. . . a few henriesÓ, not Ò. . . a few HÓ.
\item Use a zero before decimal points: Ò0.25Ó, not Ò.25Ó. Use Òcm3Ó, not ÒccÓ. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use Ò(1)Ó, not ÒEq. (1)Ó or Òequation (1)Ó, except at the beginning of a sentence: ÒEquation (1) is . . .Ó

\subsection{Some Common Mistakes}
\begin{itemize}


\item The word ÒdataÓ is plural, not singular.
\item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ÒoÓ.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ÒinsetÓ, not an ÒinsertÓ. The word alternatively is preferred to the word ÒalternatelyÓ (unless you really mean something that alternates).
\item Do not use the word ÒessentiallyÓ to mean ÒapproximatelyÓ or ÒeffectivelyÓ.
\item In your paper title, if the words Òthat usesÓ can accurately replace the word ÒusingÓ, capitalize the ÒuÓ; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ÒaffectÓ and ÒeffectÓ, ÒcomplementÓ and ÒcomplimentÓ, ÒdiscreetÓ and ÒdiscreteÓ, ÒprincipalÓ and ÒprincipleÓ.
\item Do not confuse ÒimplyÓ and ÒinferÓ.
\item The prefix ÒnonÓ is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ÒetÓ in the Latin abbreviation Òet al.Ó.
\item The abbreviation Òi.e.Ó means Òthat isÓ, and the abbreviation Òe.g.Ó means Òfor exampleÓ.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if you filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named ÒHeading 1Ó, ÒHeading 2Ó, ÒHeading 3Ó, and ÒHeading 4Ó are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation ÒFig. 1Ó, even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity ÒMagnetizationÓ, or ÒMagnetization, MÓ, not just ÒMÓ. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write ÒMagnetization (A/m)Ó or ÒMagnetization {A[m(1)]}Ó, not just ÒA/mÓ. Do not label axes with a ratio of quantities and units. For example, write ÒTemperature (K)Ó, not ÒTemperature/K.Ó

\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.



\begin{thebibliography}{99}

\bibitem{c1} G. O. Young, ÒSynthetic structure of industrial plastics (Book style with paper title and editor),Ó 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15Ð64.
\bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
\bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
\bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
\bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
\bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
\bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
\bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
\bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
\bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
\bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
\bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
\bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
\bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
\bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
\bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
\bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
\bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
\bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
\bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 






\end{thebibliography}



==> Database Cache Attack/conclusion.tex <==
%\vspace{-3mm}
\section{Conclusions and Future Work}\label{sec:conclusion}

In this work we launched a cache side-channel attack against the SQLite database management system. We developed two algorithms that approximately recover the database using the information leaked from the side-channel attack. Finally, we showed the effectiveness of closest vector problem (CVP) solvers in reducing the overall noise in the recovered databases to obtain databases with improved accuracy. We showed that for attributes with range of size $12$ our algorithm can recover the approximate database in at most $190$ seconds with \dnote{average?} maximum error percentage of $0.11 \%$. We have also extended our analysis to study the effect of heavy load on the system as well as cases where some of the ranges are missing. We have shown that the error percentage for those cases remain below $2 \%$.
\dnote{The error percentage given here is contradicting what was given earlier.}\anote{I report the number from Table 3 now.}

As a possible approach to mitigate the attacks presented in this work, we suggest that when processing a range query, a random number of dummy elements get appended to the results and returned in addition to the true matches. The effect of such a countermeasure is twofold. (1) It makes it difficult for the side-channel attacker to able to aggregate information over different runs to obtain good approximations of the volumes. (2) It makes the graph generation and clique-finding algorithms more expensive, as there will be a large number of additional nodes and edges in the graph (recall that each observed volume corresponds to a node in the graph).
Since clique-finding is NP-hard, adding even a small fraction of nodes to the graph can make the attack infeasible.

As a future work, it would be interesting to explore the effectiveness of the attack using fewer traces; in the extreme case it is interesting to study the scenario where only $1$ trace per query is given. Moreover, it would be of interest to study the performance of the Prime \& Probe ~\cite{osvik2006cache} which is a more generic type of cache side-channel attack that can be used even in scenarios where the victim and attacker do not have a shared library. Further, as mentioned previously, improved attacks on encrypted databases are possible when the full access pattern is revealed (cf. Grubbs et al.~\cite{grubbs2019learning}). It will be interesting to explore whether partial information about the access pattern can be obtained via the cache side-channel and whether this information can be used to obtain improved attacks.
We have simulated some non-uniform query distribution, and one area that can be explored more is to study what are the most realistic query distribution.
One limitation we faced in the work is the scalability of solver for NP-hard problem, i.e. clique finding algorithm. The work of Grubbs et al.~\cite{grubbs2018pump} tolerate this by having a prepossessing step. This step enables the algorithm to work even for the cases where the size of the graph is large and it is interesting to study whether a prepossessing step can be applied to cases where volumes are noisy. 
%\anote{countermeasures, show some other directions that we thought, launched side-channels and show the recovered database with some accuracy and developed a new algorithm...} 

%\dnote{Future work: Rigorous guarantees on runtime/data distributions that can be recovered? Prime \& Probe instead of Flush + Reload? Utilization of data cache and access patterns? Reconstruction of multiple columns? **Countermeasures**?} \anote{tried to fixed}






==> Database Cache Attack/experiment.tex <==
%\vspace{-3mm}
\section{Experimental Results}\label{sec:experiments}


\iffalse
In this section we describe our experimental results which were obtained by running our cache attack on SQLite on (1) random samples of a real database (2) synthetic databases with entries sampled from normal distributions. For (1), we used the NIS2008 dataset, which has xxx attributes. We initialized the database using SQLite and performed the range queries on the AMONTH attribute which corresponds to XXX.\anote{explain the database}. 
\dnote{Shouldn't the list above be consistent with this? I.e. (1) and (2) should match I, II, III. It's confusing.}
\fi

% Experiment I: Real db uniform
% Experiment II: Gaussian db uniform
% Experiment III: Noise on real db
% Experiment IV: Nonuniform Queries
% Experiment V: Missing Volumes

%We performed four sets of experiments denoted by I, II, III. 
We performed five sets of experiments. The first two experiments (I and II) are for the cases where there is no additional noise during the measurement and the query distribution over all the possible queries are uniform. The third set of experiments (III) in Section~\ref{subsec:extraload} studies the effect of extra load on the system while taking measurements. The fourth set of experiments (IV) in Section~\ref{subsec:nonuni} looks at different query distributions. In the last set of experiments (V) in Section~\ref{subsec:missingvol}, we look at the effect of missing some volumes due to the fact that some range queries may have never been issued, or due to noise causing a query to be missed entirely. 
In Experiment I, we first prepare 10 databases from the  NIS2008 database, by randomly selecting $100,000$ records. 
Nationwide Inpatient Sample (NIS) is part of the Healthcare Cost and Utilization Project (HCUP) which is used to analyze national trends in healthcare~\cite{nis2880}. The NIS is collected annually and it gathers approximately 5 to 8 million records of inpatient stays. We selected NIS from the year 2008; the full description of each attribute of the database is reported in~\cite[Table1]{nis2880}. 
In the first set of experiments we performed uniform range queries on the AMONTH attribute which corresponds to admission month coded from (1) January to (12) December (i.e., each of the possible ranges were queried with equal probability). 
In the second set of experiments (Experiment II) we sampled the database as follows: For each of the $10$ databases from Experiment I, for each record in the database, instead of using the real value for the AMONTH column, we generated synthetic data by sampling a value from a Gaussian (Normal) distribution with mean $\frac{1+N}{2} = 6.5$ and standard deviation of $3$ and $4$, respectively. So within Experiment II, we considered two data distributions, a ``narrow'' Gaussian with standard deviation $3$ and a ``wide'' Gaussian with standard deviation $4$. 

%Later in this section, we also present the performance of Error Reduction Step by using CVP.

We ran the experiments on a Lenovo W540 Laptop with Intel Core i7-4600M CPU clocking at $2.9$ GHz running Ubuntu 16.04. The L1, L2 and L3 caches have capacities 32KB, 256KB and 4MB, respectively. For the SQLite, we use the amalgamation of SQLite in C, version 3.20.1.
We heuristically observed that if we gather around $120$ measurements for any one range query, the aggregated side-channel measurements will result in a peak corresponding to the approximate volume.
Since there are at most $78$ different range queries for $N=12$ we decided to gather around $10,000$ traces to make sure there are enough traces for each range to be able to see a peak for each approximate volume.

We gathered $10,000$ traces corresponding to $10,000$ uniformly chosen range queries for Experiments I and II, i.e. $1$ trace for each query. We processed all those traces to obtain the approximate/noisy volumes. On average, gathering $10,000$ traces takes around $8$ hours and processing them takes another $3$ hours. The experiments and the code to run the Clique-finding algorithm, Match \& Extend and noise reduction step can be found here~\cite{github:repo}.

After processing the measurements, we obtained a set of approximate volumes, on which we then ran noisy clique-finding and Match \& Extend, which in turn output reconstructed databases. Figure~\ref{fig:exp1} illustrates the quality of the recovered values for the noisy clique-finding and Match \& Extend algorithms. 
The noisy clique-finding algorithm is run with several values for the noise budget while the Match \& Extend is run with a fixed noise budget of $0.002$. 
For each of the $N$ values $1, 2, \dots, N$, we expect to recover a candidate volume, corresponding to the number of records in the database that take that value. 
For a database with range of size $N$, we define the success rate as the number of candidate volumes recovered divided by $N$. 
For example in our experiments if we recover only $11$ candidate values for a database of range of size $N = 12$, then we have a success rate of $11/12$. It is also worth mentioning that the attacker can distinguish a successful attack from the failed one, since $N$, i.e. the size of the range, is known to the attacker. 
\mnote{changed the wording of Error Rate definition below}
We define the error rate of a recovered volume as its percentage of deviation from the original volume that it corresponds to.
% For the error rate, 
We look at the recovered database and compare it to the original one. For each candidate volume $v'$ that is recovered, we compare it to the corresponding value in the real database, $v$ and report the error rate as $\left(\frac{|v'-v|}{v}\right) \times 100$.
%Note that in some cases less than $N$ candidate volumes were recovered, and we simply omit those from the computation of the average error rate.
%If there are $N$ values recovered, we just have to check which of the recovered database or the mirror of that is closer to the original database. If we only recover less than $N$ coordinates we then try to align those with the real database to get the closest answer. Then we compute the percentage that the values are off in each location.
\dnote{I don't understand the sentences above starting from ``For the Error Percentage.'' Tried to fix.}\anote{fixed}
So for example, if a recovered volume is $7990$ and the actual volume was $8000$ we report an error percentage of $0.12 \%$. 
If the algorithm only recovered $11$ values for a database of size $12$,
%we manually find the best match and for each of those $11$ locations and 
we will report the percentage error for the $11$ recovered values. 

Figure~\ref{fig:exp1} and~\ref{fig:exp2} show both the success rate and the error percentage for Experiment I and II. For \textit{success rate} (orange line), it can be seen that for the noisy clique-finding algorithm, increasing the noise budget helps to recover more volumes in both experiments.
The Match \& Extend algorithm, used with a fixed noise budget of $0.002$ could recover all the volumes in both of the experiments. 
\dnote{I don't understand the previous sentence.}\anote{tried to fix}
For \textit{error percentage} the average percentage of error is marked with a blue dot. The $90\%$ confidence interval is marked with the black marker. 
The confidence interval indicates that for a new set of experiments with the same setting, we are $90 \%$ confident that the average error rate will fall within that interval. \anote{tried to explain the $90 \%$ confidence interval and it needs better explanation} For the noisy clique-finding algorithm, increasing the noise budget causes the average error percentage to increase and the confidence interval to grow. 
\mnote{reworded the following sentence (original version commented)}
In some cases with noise budget $0.005$ and $0.006$, some of the recovered databases in Experiment I were very far off from the actual databases, causing the error interval in these settings to be much larger than in other settings.
% There are some cases for noise budget $0.005$ and $0.006$ in Experiment I, in which the error interval is much larger than the others.
% \dnote{I don't understand the above sentence.}\anote{fixed}
% Those cases correspond to recovered databases that have some values which were completely off compared to the correct values of the actual database.

%In these cases the noisy clique-finding algorithm recovered a database which had very poor accuracy in a few locations causing the error interval to grow. 
In a nutshell, although it seems that increasing the noise budget helped to achieve higher success rates, since the error percentage grows, the quality of the recovered databases is lower. 
For the Match \& Extend algorithm the average amount of error and the width of error interval is comparable to the noisy clique-finding algorithm with small noise budget but the success rate is much higher. 
Figure~\ref{fig:exp1-2_runtime} shows the average run time as well as $90 \%$ confidence interval 
%(as it was explained in the above) 
of the successful database recovery in seconds.
\dnote{I don't understand what you mean by $90\%$ confidence?}\anote{tried to fixed}
It can be seen that the average run time of noisy clique grows with the size of the noise budget. The Match \& Extend algorithm, however, always uses noise budget of $0.002$ and so its average running time remains low.

\begin{figure*}[h]
\centering
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/real_db_perf.pdf}
\subcaption{Success Rate and error percentage for Experiment I}
\label{fig:exp1}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/gauss_db_perf.pdf}
\subcaption{Success rate and error percentage for Experiment II}
\label{fig:exp2}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.3\textwidth}
\includegraphics[width=\textwidth]{figures/run_time.pdf}
\subcaption{Average running time of Noisy Clique for different Noise Budget vs. Match \& Extend Algorithm}
\label{fig:exp1-2_runtime}
\end{subfigure}
%

\caption{(a),(b) Comparison of the Success rate and Error Percentage for the noisy clique algorithm and Match \& Extend algorithm. The noisy clique algorithm is run using noise budget in the range $0.001-0.006$ and Match \& Extend is run with noise budget $0.002$. The orange line is the success rate (higher is better). The blue dot is the average error percentage and the black line segment is the $90\%$ confidence interval (lower dot and narrower interval is better).
(c) Average running time of Noisy Clique for different Noise Budget vs. Match \& Extend Algorithm with Noise Budget of $0.002$. 
%The black line shows the $90\%$ confidence interval.
\dnote{I don't understand what you mean by $90\%$ confidence?}
\mnote{this definition of the confidence interval was given before. I believe we can remove from here?}\anote{added in text}}
\label{fig:exp_all}
\end{figure*}


\iffalse
\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{figures/real_db_perf.png}
\caption{Success Rate and error percentage for Experiment I}
\label{fig:exp1}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{figures/gauss_db_perf.png}
\caption{Success Rate and error percentage for Experiment II}
\label{fig:exp2}
\end{figure}
\fi

\iffalse
\begin{figure*}[h]
\centering
\begin{subfigure}[t]{0.30\textwidth}
\includegraphics[width=\textwidth]{figures/real_db_perf.png}
\subcaption{Success Rate and error percentage\\ for Experiment I}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.30\textwidth}
\includegraphics[width=\textwidth]{figures/nonuni_db_perf.png}
\subcaption{Success rate and error percentage\\ for Experiment II}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.30\textwidth}
\includegraphics[width=\textwidth]{figures/gauss_db_perf.png}
\caption{Success rate and error percentage\\ for Experiment III}
\end{subfigure}
%

\caption{Comparison of the Success rate and Error Percentage for the noisy clique algorithm and Match \& Extend algorithm. The noisy clique algorithm is run using noise budget in the range $0.001-0.006$ and Match \& Extend is run with noise budget $0.002$. The orange line is the success rate (higher is better). The blue dot is the average error percentage and the black line segment is the $90\%$ confidence interval (lower dot and narrower interval is better).\dnote{I don't understand what you mean by $90\%$ confidence?}
\mnote{this definition of the confidence interval was given before. I believe we can remove from here?}\anote{added in text}}
\label{fig:exp_all}
\end{figure*}
\fi


\iffalse
%\anote{non-uniform query failed completely failed on one database but uniform gives something which was off, the success rate can be seen in Figure 8} 
\begin{figure}[t]
 \centering
  \includegraphics[width=0.8\linewidth]{figures/run_time.png}
  \caption{Average running time of Noisy Clique for different Noise Budget vs. Match \& Extend Algorithm with Noise Budget of $0.002$. The black line shows the $90\%$ confidence interval.}
  %The confidence interval represents that for a new set of experiments with the same setting we are $90 \%$ confident that the average running time will be in the marked interval. \dnote{I don't understand what you mean by $90\%$ confidence?}\anote{added}}
  \label{fig:run_time}
\end{figure}
\fi

\begin{table}[]
\caption{Performance Comparison of Noisy Clique with Noise Budget $0.006$ vs. Match \& Extend Algorithm, with $99\%$ Confidence interval}
\footnotesize
\begin{tabular}{c|c|c|}
\cline{2-3} & \begin{tabular}[c]{@{}c@{}}Noisy Clique\\ (0.006)\end{tabular} & Match \& Extend \\ \hline
\multicolumn{1}{|c|}{Error Percentage} & 0.10 \% - 0.27 \% & 0.07 \% - 0.11 \% \\ \hline
\multicolumn{1}{|c|}{Run Time (s)} & 0 - 1900 & 38 - 190\\ \hline
\end{tabular}
\label{tab:perf}
\end{table}


Table~\ref{tab:perf} compares the performance of the Match \& Extend algorithm and the noisy clique algorithm on successful instances (meaning, the performance of the noisy-clique is taken only over the instances for which the recovered database had the correct size $N$). \dnote{I took this out, I don't think that's what you mean... ``with the same success rate.''}
The noisy clique-finding algorithm with noise budget $0.006$ performs better in terms of success rate than noisy clique-finding with smaller noise budgets, and we select it as a comparable algorithm to Match \& Extend algorithm. We are $99 \%$ certain that in a new set of experiments with the same setting as presented here, the Match \& Extend algorithm would output a result in at most $190$ seconds with at most $0.11 \%$ error. The noisy clique finding algorithm, on the other hand, would output a result in at most $1900$ seconds with at most $0.27 \%$ error. We have also analyzed the effect noise reduction step to further reduce the noise, which can be found in Section~\ref{sec:cvp_res}.



%\vspace{-3mm}
\subsection{Additional Noisy Process Running}\label{subsec:extraload}

For Experiment III, we extend our analysis to the case where there is extra load on the system---i.e.~extra processes running---during the time of the attack. To run the noisy processes we use the command \texttt{stress -m i}, where $i$ represents the number of parallel threads running with CPU load of $100 \%$. We repeat the experiment for $i \in \{1,2,8\}$ and present the results in Figure~\ref{fig:noisy_process}. We took $5$ databases from Experiment I and obtained new sets of traces while the system had noisy processes running at the background. We recovered all the coordinates of the databases for all cases, so the success rate for all cases remains at $100 \%$. The quality of the recovered databases worsened with heavier loads, however even with $8$ noisy processes the average error remains less than $2 \%$. 

\begin{figure}[t]
 \centering
  \includegraphics[width=0.8\linewidth]{figures/noisy_process.pdf}
  \caption{Success Rate and error percentage for Experiment III. The system is analyzed under different varying load. The load is increased by adding extra 1,2,8 processes. 
  %The orange line is the success rate (higher is better). The blue dot is the average error percentage and the black line segment is the $90\%$ confidence interval (lower dot and narrower interval is better).
  }
  \label{fig:noisy_process}
\end{figure}
\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.30\textwidth}
\includegraphics[width=\textwidth]{figures/nonuni_db_perf.pdf}
\subcaption{Success Rate and error percentage for Experiment IV}
\label{fig:nonuni}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.30\textwidth}
\includegraphics[width=\textwidth]{figures/missing_vols.pdf}
\subcaption{Success rate and error percentage for Experiment V 
%when some of the queries are not made
}
\label{fig:missingvols}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.30\textwidth}
\includegraphics[width=\textwidth]{figures/missing_big_vols.pdf}
\caption{Success rate and error percentage for Experiment V
%when large query sizes are blocked
}
\label{fig:missingbigvols}
\end{subfigure}
%

\caption{Performance of Match \& Extend algorithm in different cases (a) non-uniform query (b) Missing Volumes (c) Queries with large response size are blocked. The orange line is the success rate (higher is better). The blue dot is the average error percentage and the black line segment is the $90\%$ confidence interval (lower dot and narrower interval is better).
}
\label{fig:exp_all_noisy}
\end{figure*}

%\vspace{-3mm}
\subsection{Non-uniform Query Distribution}~\label{subsec:nonuni}
As mentioned, in order to be able to detect an approximate volume in our side-channel measurements, we need to observe at least $120$ measurements per range query. 
While we require that each query must be made some minimum number of 
times,
we do not impose that the query distribution must be uniform.
This is in contrast to previous work by Kellaris et al.~\cite{kellaris2016generic} who crucially required uniform query distribution. Our requirement can be seen as the noisy analogue of Grubbs et al.~\cite{grubbs2018pump}, who required each volume to be observed at least once in the \emph{noiseless} setting. To tolerate the noise present in the measurement in our setting, we require each query to be observed at least $120$ times. Later, in Subsection~\ref{subsec:missingvol}, we will further relax this requirement by showing that the recovery can be done even if some of the range queries are entirely omitted. This can be viewed as a weakening of even the requirements of Grubbs et al.~\cite{grubbs2018pump}.

For Experiment IV, we used the same databases as in Experiment I, but performed non-uniform range queries. We picked $5$ database from Experiment I and tested them with $3$ sets of non-uniform query distributions 
which results in $15$ scenarios in total. 
The first query distribution is chosen based on the assumption that queries of the form $\range{i}{i+1}$ are made twice as often as the other queries. The second query distribution assumed that queries in the form of $\range{i}{i+1}$ and $\range{i}{i+2}$ are made twice as often as the other queries. For the last query distribution, we tested the hypothesis that the determining factor for our attack seems to be the ability to identify ``peaks'' that roughly correspond to the volumes of the range queries (e.g.~see Figure~\ref{fig:volume_attack} and Figure~\ref{fig:aprox_vs_real}). A challenging query distribution is therefore one which causes one of the peaks to disappear as the peak adjacent to it dominates it. To test our hypothesis, we chose a distribution in which range $[a,b]$
was queried twice as often as 
$[c,d]$ when ranges $[a,b]$ and $[c,d]$ had
close volumes (and therefore close peaks). 

Figure~\ref{fig:nonuni} shows both the success rate and the error percentage for Experiment IV. It can be seen that the noisy clique-finding algorithm exhibits better success rate as the noise budget increases, while the error percentage grows as well. Match \& Extend algorithm, however has $100 \%$ success rate with low error percentage. We have also analyzed the effect of the noise reduction step to further reduce the noise, which can be found in Section~\ref{sec:cvp_res}. 

%Specifically, in these experiments we either queried the first half of the possible ranges twice as often as the second half or vice versa.
% In Experiment II, we gathered up to $15,000$ traces so we would have enough observations for the queries which are made fewer times.
% In Experiments II, however, we did not observe volumes which were completely off for noise budget $0.005$ and $0.006$ but as it can be seen the success rate did not reach $100 \%$. So the noisy clique-finding algorithm completely failed for some instances.

%\vspace{-3mm}
\subsection{Missing Queries}~\label{subsec:missingvol}

\iffalse
\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{figures/nonuni_db_perf.png}
\subcaption{Success Rate and error percentage for Experiment IV}
\label{fig:nonuni}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{figures/missing_vols.png}
\subcaption{Success rate and error percentage for Experiment V 
%when some of the queries are not made
}
\label{fig:missingvols}
\end{subfigure}
%
\hfill
\begin{subfigure}[t]{0.25\textwidth}
\includegraphics[width=\textwidth]{figures/missing_big_vols.png}
\caption{Success rate and error percentage for Experiment V
%when large query sizes are blocked
}
\label{fig:missingbigvols}
\end{subfigure}
%

\caption{Performance of Match \& Extend algorithm in different cases (a) non-uniform query (b) Missing Volumes (c) Queries with large response size are blocked.
%The orange line is the success rate (higher is better). The blue dot is the average error percentage and the black line segment is the $90\%$ confidence interval (lower dot and narrower interval is better).
}
\label{fig:exp_all_noisy}
\end{figure*}
\fi

For Experiment V, we study the performance of our algorithm when some of the ranges are never queried. We consider two cases. In the first case, we look at a setting in which certain randomly chosen ranges
%\newnote{Is that correct?}
are never queried and in the second case, we consider a setting in which the queries corresponding to the largest volumes are never made. For the first case, we randomly drop $\{1,2,4,6,8\}$ volumes from the measurements. The performance of Match \& Extend algorithm can be seen in Figure~\ref{fig:missingvols}. As more and more volumes are dropped, the success rate of the algorithm decreases. For example, in the case where $8$ volumes are missing we recovered around $95 \%$ of the databases entries. However, the error percentage grows as more and more volumes are missing, although it remains below $1 \%$ error even for the case where $8$ volumes are missing. For the second case, we first look at the case where the query $\range{1}{N}$ is blocked, i.e.~the attacker is not allowed to query the whole database. In other cases the queries which ask for more than $90 \%, 80 \%$ and $70 \%$ of the database is blocked, respectively. It can be seen in Figure~\ref{fig:missingbigvols} that in these cases the success rate remains around $98 \%$ and the error percentage of the recovered coordinates stays below $2 \%$. 




\iffalse

Figure~\ref{fig:noise_budget_me} shows the performance of the clique finding algorithm as well as the Match \& Extend algorithm. In all the experiments we run the attack and assess whether we recovered a database with $N$ values. If we recover a database of size $N$, we regard that experiments as successful. As it can be seen, In the initial experiment with noise budget of $0.003$ there are $5$ experiments which are successful in the experiments I, II but all the experiments III failed. As we increases the noise budget to $0.004$ there are more experiments working in all experiments I, II and III, however not all of them were successful. Once we ran Match \& Extend algorithm with noise budget $0.002$ all the experiments were successful.

\begin{figure}
 \centering
  \includegraphics[width=0.8\linewidth]{figures/noise_budget_me.pdf}
  \caption{Caption}
  \label{fig:noise_budget_me}
\end{figure}


We compute the absolute value of the amount that each database entry is off from the correct value. We set the noise budget equal to $0.004$ for the clique experiments and the noise budget is set to $0.002$ for the Match \& Extend algorithm. We report how many each entry is off for all three sets of experiments. The green bar shows the bar plot obtained from the clique algorithm, and the blue bar shows the value for Match \& Extend algorithm. As it can be seen the curve which was fitted to the clique is wider, while the curve fits to Match \& Extend algorithm is narrower and closer to zero. This shows that the recovered value from the Match \& Extend algorithm is closer to the correct values. 

\begin{figure}
 \centering
  \includegraphics[width=0.8\linewidth]{figures/curves.pdf}
  \caption{\anote{here ...}}
  \label{fig:curves}
\end{figure}


\fi


%To perform the attacks, the victim and attacker are run in parallel. The victim issues range queries to the database while victim is monitoring the cache lines. 

%\subsection{Observing All Queries} For this section 


%\subsection{Missing Volumes}


\iffalse
In this section we describe the experimental results which are constructed both from synthetic data as well as data gathered from running cache attack on sqlite.

\dnote{Sections can be, in order: ``Cache-Side Channel Attack on Synthetic Data,'' ``Cache-Side Channel Attack on Real Data,''
``Auxiliary Information on Query Distribution,'' ``Auxiliary Information on Data Distribution,'' ``Attacks on Synthetic Data and Noise.''}

%\subsection{Synthetic Data}
%\dnote{This section should go \emph{last} since it is only relevant due to the differential privacy connection and is not the main focus of our paper. The main focus of our paper is the cache attack.}



%\subsection{Cache-Side Channel Attack on Real Data}



\subsection{Cache-Side Channel Attack on Synthetic Data}

For these experiment the recovered volume will be duplicated to take into account the potential duplication in volumes. For this part $5$ sample instance of database is created. To construct the database we sample $1000$ entries uniformly at random from the range $1$ to $15$ and the approximates volumes are recovered by cache side-channel. The result of experiments are presented in Table~\ref{tab:duplicate} and for each algorithm we report the $L2$ distance of reconstructed database from the correct one. As it can be seen in Table~\ref{tab:duplicate} The combination of subgraph isomorphism and CVP reconstructs databases which are closer to the correct database. 

\begin{table}[]\label{tab:duplicate}
\centering
\begin{tabular}{|c|cccc|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Column\\Distribution\end{tabular}} & \multicolumn{1}{c|}{Instance \#} & \multicolumn{1}{c|}{Clique} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Subgraph \\Isomorphism\end{tabular}} & \multicolumn{1}{c|}{CVP} \\ \hline
\multirow{5}{*}{Uniform} 
    & 1 & 1.41 & 1.41 & 1.41 \\
    & 2 & 4.24 & 2.24 & 2.24 \\
    & 3 & 4.58 & 2.24 & 2.0 \\
    & 4 & 3.0 & 1.73 & 1.73 \\
    & 5 & 4.06 & 3.16 & 3.16 \\ \hline
\end{tabular}
\caption{The recovered volumes are duplicated and target graph is constructed as explained in Section~\ref{sec:subgraph_iso_noiseless}. For each algorithm the $L2$ distance of the reconstructed volume from correct database is reported.}
\end{table}

\subsection{Auxiliary Information on Query Distribution}

As it was explained in Section~\ref{sec:aux_query}, only the volume which occurs more frequent than their neighbours are duplicated. We ran $3$ different experiments and for each experiment we sample $1000$ entries for the database, in the first one each entry is sampled uniformly at random from range $1$ to $15$. For the non-uniform case, we consider two cases which are once the data is coming from Gaussian distribution with small standard deviation i.e. ``Narrow'' and the second case where data is coming from Gaussian with larger standard deviation i.e. ``Wide''. In both cases the mean of Gaussian is set to $\frac{15}{2} = 7.5$. For each case, the $L2$ distance of reconstructed database from correct database is reported in Table~~\ref{tab:auxquery} and for this scenario, the combination of subgraph isomorphism and CVP gives closer answer to the correct database. 

\begin{table}[]\label{tab:auxquery}
\centering
\begin{tabular}{|c|cccc|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Column\\Distribution\end{tabular}} & \multicolumn{1}{c|}{Instance \#} & \multicolumn{1}{c|}{Clique} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Subgraph \\Isomorphism\end{tabular}} & \multicolumn{1}{c|}{CVP} \\ \hline
\multirow{5}{*}{Uniform} 
    & 1 & 1.41 & 1.41 & 1.0 \\
    & 2 & 2.0 & 2.65 & 1.41 \\
    & 3 & 6.63 & 1.41 & 1.73 \\
    & 4 & - & - & - \\
    & 5 & 6.63 & 3.16 & 2.45 \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Narrow \\ Gaussian\end{tabular}}
    & 1 & 1.0 & 1.0 & 1.0 \\
    & 2 & 73.88 & - & - \\
    & 3 & 1.0 & 1.0 & 1.0 \\
    & 4 & - & - & - \\
    & 5 & 1.73 & 1.41 & 1.41 \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Wide \\ Gaussian\end{tabular}}
    & 1 & 3.32 & 2.24 & 1.41 \\
    & 2 & 1.41 & 1.41 & 1.0 \\
    & 3 & 0.0 & 1.0 & 0.0 \\
    & 4 & 1.41 & 0.0 & 1.41 \\
    & 5 & 2.55 & 0.0 & 0.0 \\ \hline    
\end{tabular}
\caption{$L2$ of reconstructed databases for the case where Auxiliary Information on Query Distribution is given for $N = 15$}
\end{table}

\subsection{Auxiliary Information on Data Distribution}

Similar to previous case we consider wide and narrow Gaussian. The range of database $N = 15$ and each database has $1000$ entries and the volume are recovered using cache side-channel attacks. The recovered volumes are duplicated (to catch the cases where there are equal volumes from different ranges) and the construction of the target and pattern graph is described in Section~\ref{sec:aux_data}. We ran $5$ different experiment and for each experiment we measure the $L2$ distance of the result from correct database. Table~\ref{tabl:aux_info_data} presents the results and it can be seen that by using the auxiliary information the recovered databases are close to the actual one. It is worth mentioning that in this scenario, we can get an ``approximate'' database without running any attack at all by just sampling from the data distribution. However, in this case each entry of the real database is likely to deviate by $\pm \alpha \cdot \sigma$ in each entry. Whereas it can be seen in Table~\ref{tabl:aux_info_data}, that our attack allows us to achieve nearly exact reconstruction of the database.  

\dnote{Explain that in this case, we can get an ``approximate'' database without running any attack at all. However, in this case each entry of the real database is likely to deviate by $\pm \alpha \cdot \sigma$ in each entry. On the other hand, our attack allows us to achieve nearly exact reconstruction of the database.}\anote{just compied the above statement}

\begin{table}[]\label{tabl:aux_info_data}
\centering
\begin{tabular}{|c|ccc|}
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Column\\Distribution\end{tabular}} & \multicolumn{1}{c|}{Instance \#} &  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Subgraph \\Isomorphism\end{tabular}} & \multicolumn{1}{c|}{CVP} \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Narrow \\ Gaussian\end{tabular}} 
    & 1 & 1.41 & 0.0 \\
    & 2 & 2.24 & 1.73 \\
    & 3 & 0.0 & 0.0 \\
    & 4 & 2.29 & 1.41 \\
    & 5 & 2.24 & 2.23 \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Wide \\ Gaussian\end{tabular}}
    & 1 & 3.32 & 2.0 \\
    & 2 & 1.73 & 1.0 \\
    & 3 & 1.73 & 1.73 \\
    & 4 & 1.0 & 1.0 \\
    & 5 & 2.0 & 1.87 \\ \hlinehttps://www.overleaf.com/4192949652cgjtwbcxtqgt
\end{tabular}
\caption{Each instance is a database of size $1000$ with $N=15$. The target graph ans pattern graph are constructed using auxiliary information. For each instance the $L2$ distance of the recovered database from actual database is reported.}
\end{table}


\subsection{Attacks on Synthetic Data and Noise}
We start by looking into the noisy volumes. The scenario we are considering is to add Gaussian noise to each volume to perturb each of them by small value. To be specific assuming there are $\binom{N}{2} + N$ nodes in the perfect scenario. In the noisy case we perturb the value of each nodes by small values by adding a Gaussian noise to each value. The target graph is constructed as mentioned in Section~\ref{sec:target_graph}. We reconstruct the database using two method. In the first approach we use clique finding algorithm and in the second method we use the subgraph isomorphism approach along with CVP to further reduce the noise. In both approaches we report the $L2$ distance of the final result from the correct database. \anote{needs better wording - might not be necessary at all though}As a note the $L2$ norm of the final solution has be within a bound of the error. 


Figure~\ref{fig:dist_uniform} shows the distribution of $L2$ distance of recovered database from the actual database in the case where the actual database has uniform distribution. Each value of the volume is perturbed by adding noise from Gaussian distribution with standard deviation $0.2$. We ran this experiment for total of $214$ times and for each run we created $100$ different permutation of target graph. Subgraph isomprhism and CVP could output an answer in total of $207$ times and clique outputed in $205$ times. However, as it can be seen the $L2$ distance of solutions which are outputted by subgraph isomporphism and CVP are smaller than that for clique, which means that the solution outputed by subgraph isomprhism are ``closer'' to correct database. 

\begin{figure}
 \centering
  \includegraphics[width=0.9\linewidth]{figures/dist_uniform.pdf}
  \caption{Performance comparison of three reconstruction approach when the column of the database has uniform distribution and each volume is perturbed by adding a noise based on Gaussian distribution with standard deviation of $0.2$. We ran $214$ experiments in total. Subgraph isomprhoism and CVP output an answer in $207$ times and clique output an answer $205$ times.}
  \label{fig:dist_uniform}
\end{figure}

Figure~\ref{fig:dist_gauss} shows the $l2$ distance of the recovered database from the actual database for the case where the database is sampled from Gaussian distribution. Similar to previous case, each value of the volume is perturbed by adding noise from Gaussian distribution with standard deviation $0.2$. We ran this experiment for total of $1181$ times and for each run we created $100$ different permutation of target graph. Subgraph isomprhism and CVP could output an answer in total of $46$ times and clique outputed in $1178$ times. However, It can be seen than clique solver outputs results which are significantly further than actual database comparing to solution outputted by subgraph isomorphism solver. 

\anote{One thing which is not shown in this figure is there was multiple instance where subgraph isomorphism could not find an answer in reasonable amount of time so we don't consider those cases in this figure, should we add the previous sentence as well?}
\dnote{Yes, of course. This is crucial to include! We should think about how to resolve this problem.}
 
\begin{figure}
 \centering
  \includegraphics[width=0.9\linewidth]{figures/dist_gauss.pdf}
  \caption{Performance comparison of three reconstruction approach when the column of the database has Gaussian distribution and each volume is perturbed by adding a noise based on Gaussian distribution with standard deviation of $0.2$. We ran $1181$ experiments in total. Subgraph isomprhoism and CVP output an answer in $46$ times and clique output an answer $1181$ times.}
  \label{fig:dist_gauss}
\end{figure}







% Please add the following required packages to your document preamble:








%\subsection{Results for Cache Attack with Auxiliary Information on Query Distribution}

%\subsection{Results for Cache Attack with Auxiliary Information on Data Distribution}

%\dnote{Explain that in this case, we can get an ``approximate'' database without running any attack at all. However, in this case each entry of the real database is likely to deviate by $\pm \alpha \cdot \sigma$ in each entry. On the other hand, our attack allows us to achieve nearly exact reconstruction of the database.}

\fi

==> Database Cache Attack/introduction.tex <==
\section{Introduction}

\iffalse
\dnote{Consistency in naming algortihms:
\begin{itemize}
    \item \emph{noisy} clique-finding
    \item Extend vs.~Match \& Extend.
    Also, is this an algorithm that gets run
    in addition to noisy clique-finding
    or instead of noisy clique-finding?
    \item Should we name the CVP part as well? E.g. ``error reduction step.''?
\end{itemize}}
\anote{We have two main algorithm one is \emph{noisy} clique-finding and in addition to that we have the second step called ~Match \& Extend. There should not be any explain algorithm anymore as we decided to change explain to \emph{Match \& Extend}. I will have that in mind in pass to make sure it is consistent. Also I agree we can call CVP ``error reduction step.''}
\fi
\dnote{Major things to do:
\begin{itemize}
    \item Section on "Assessing effectivenss of previous algorithms.."
    \item section on "Overview of Experimental Results."
    \item Experimental Section
    \item Conclusions section. We should probably say something about countermeasures there.
    \item Make sure we have included all the related work and given credit.
    \item Add claims (or revisit claims we already make) on run-time and/or uniform vs. non-uniform queries.
    \item Make sure all comments addressed
\end{itemize}
}
\anote{"Assessing effectivenss of previous algorithms.." and "Overview of Experimental Results." needs a pass}
\anote{Experimental Section }
\anote{run time of the algorithm grows exponentially with size of range but not with size of database, the NP-hard part regarding the clique}
\anote{conclusion is done}

%\textbf{Motivation:} 
%\dnote{Aria: please polish this section. We can't simply write statements like ``lots of private data is being outsourced to the cloud.'' This needs to sound like an academic paper.}
%Talk about how lots of private data is being outsourced to the cloud. 
%Importance of exploring attack space in order
%to enable the development of targeted countermeasures. Importance of side-channel attacks--practicality of the attacks and the basic idea of how information gets passed from victim to spy. Main goal of our work is to develop practical attacks on typical data processing software. Explore the extent to which typical data processing tasks are susceptible to side-channel attacks.
%Launch our attacks on SQLite, which is widely used in practice. SQlite is a C-language library that implements a small and fast SQL database engine.


\iffalse
\begin{itemize}
    \item Data processing on public cloud computing services has become continually more pervasive and is now intrinsic to the business model of many sectors. Even the department of defense is using cloud computing. Indeed, AWS has established supposedly more secure versions of their clouds for DoD use.
    \item Data processing on public clouds raises important security challenges that are unique to this setting.
    \item A strong threat model is to assume that the cloud server itself is corrupted. In this case, data must be encrypted. This has been addressed via various tools in various prior works. Unfortunately, very large number of attacks are known in this setting and this has been the focus of much research. Cite papers and explain (at least for one or two of them) what information they are able to reconstruct.
    \item A weaker threat model is to assume that the server is trusted, but that a spy process has access to side-channel information about the computation of the victim in the cloud.
    \item Discuss side-channels. Discuss cache attacks.
    \item Previously side-channel/cache attacks were mainly focused on recovering cryptographic keys during computation of specific implementations of cryptographic protocols. Give examples--AES, RSA.
    \item Our goal is to explore the effect of side-channels on typical data processing, using standard open-source software. Emphasize that no cryptography at all is being used here. 
    \item Discuss SQLite and how widespread the usage of SQLite is.
    \item We consider the problem of database reconstruction. Describe problem and cite papers that have considered the same problem.
    \item Discuss one approach for database reconstruction, which is to obtain volumes of range queries. Cite papers that have considered this approach.
    \item Explain that we can use side-channels to get approximate volumes of range queries. This is done by finding an appropriate line of code that gets called for each record of the database within the range. Tracking how many times that line of code got called by the victime via a cache side channel attack.
    \item Explain why the previous attacks don't work in our setting (they crucially require exact volumes, our setting is ``noisy''). 
    \item In our work we develop new algorithmic approaches to solving the problem of database reconstruction from ``noisy'' volumes. Our basic approach is to reduce our problem to other computational problems that are well-studied in the literature and for which highly optimized solvers have been developed.
    \item One limitation of our work is that our approach uses solvers for NP-hard problems as subroutines. The complexity of these NP-hard problems grows with the size of the range. This is in contrast to the recent work of Kenny Patterson and his group which showed how to do ``approximate reconstruction'' in a way that scales only with the desired accuracy level and not the range size. Nevertheless, our results work well in practice for ranges up to size 15.
    \item We present attacks in various scenarios: Synthetic Data + Real Side Channel, Real Data + Real Side Channel, Auxiliary information, Synthetic noise (elaborate on each setting). In each setting we show that our attack is practical for databases of size up to ** and ranges of size up to **. We get accuracy of ** in each setting. Explain that when database size grows beyond ** the noise from the cache side-channel attack becomes too large.
\end{itemize}
\fi
Data processing in the cloud is becoming continually more pervasive and cloud computing is intrinsic to the business model of various popular services such as Microsoft's Office 365, Google's G suite, Adobe Creative Cloud or financial services such as intuit~\cite{cloudservices}.
Besides for cloud usage by industry, 
federal agencies are now utilizing cloud services,
even for storage and analytics of sensitive data.
For example, Microsoft recently won a $\$10$ billion government contract from the Department of Defense (DoD) to create a ``secure cloud'' for the Pentagon~\cite{DoDJedi}.
While providing important functionality, processing of sensitive information in the cloud raises important security challenges. In the extreme case, one may not trust the cloud server itself to handle the sensitive data, corresponding to a threat model in which the cloud server is assumed to be malicious. In this case, data must be encrypted, which raises the challenging task of computation over encrypted data. Techniques and tools for computation over encrypted data have been addressed in a myriad of papers~\cite{popa2011cryptdb, boldyreva2011order, lewi2016order, cash2013highly} and various privacy attacks have also been exhibited~\cite{naveed2015inference, kellaris2016generic}. 
%\dnote{removing to make more room.}
%For example in the work of Naveed et al.~\cite{naveed2015inference} it is shown how to recover the plaintext from the deterministic and order-preserving encryption by using the encrypted column and publicly available information.
%\anote{Cite papers and explain (at least for one or two of them) what information they are able to reconstruct.}\anote{done}
A weaker threat model, considered in this work, assumes that the server may be trusted to handle the sensitive data (e.g. a privacy agreement has been signed with the cloud service), but that a spy process is running on the same public server. 
If a spy process is co-located with the victim on the same physical machine they will share hardware such as a cache, which serves as a side channel. 
\iffalse
: The spy process monitors a specific cache line and measures the time it takes to access that line.
If the victim process accessed the monitored cache line, the spy's access time will be short, whereas if the victim process did not access the cache line, the spy's access time will be long. Thus, a timing attack can be launched to determine whether or not the victim process accessed a certain cache line within a period of time. 
\fi
\iffalse
Cache side-channel attacks were introduced by Tsunoo et al.~\cite{tsuno_cache} that shows a timing attack on MISTY1 block cipher.
Later, Osvik et al.~\cite{osvik2006cache} presented an attack that allowed the extraction of AES keys.

%Most other prior work on cache side-channel attacks also focus on the cryptographic setting: The goal is to recover cryptographic keys by launching cache attacks on specific implementations of cryptosystems.

Ristenpart et al.~\cite{ristenpart2009hey} demonstrated the possibility of launching cache side-channel attacks in the cloud (as opposed to on a local machine) and they pointed out that such vulnerabilities leak information about the victim VM. 
%In their paper, the spy VM must arrange to be co-located with a victim VM on the same physical machine in the cloud. They showed how to estimate with high probability where a target VM resides and then showed how to detect if they are co-located or not.
Subsequent work showed how the cache side-channel can be used to extract cryptographic keys for ElGamal~\cite{zhang2012cross}, AES~\cite{irazoqui2014wait}, RSA~\cite{184415} and recently BLISS~\cite{bruinderink2016flush} (a lattice-based signature scheme).
\fi
%Our goal is to explore the effect of side-channels on typical data processing using standard, open-source software. %where \emph{no cryptography} is involved \lnote{We don't really care whether the data are encrypted because in our threat model we have no way of reading the data.}.

Our goal is to explore the effect of side-channels on open-source database engines. We present an attack on SQLite, a C-language library that implements a small and fast SQL database engine and is among the top ten databases in the ranking released by db-engines.com.
Our threat model assumes that an external user queries a private database stored on a victim VM, upon which the victim VM processes the query using SQLite and returns the result to the external user. The attacker is disallowed from directly querying the database or observing the outputs of a query. Since the attacker is running a spy VM co-located with the victim VM in the cloud,
%The attacker sees neither the external users' queries nor the responses they receive.
it can monitor the shared cache to obtain side-channel leakage. The goal of the attacker is to reconstruct the column upon which the victim is making range queries.

%\vspace{-5mm}

\paragraph{Relationship to attacks on Searchable Encryption.}
Our work is inspired by the line of works of
Kellaris et al.~\cite{kellaris2016generic},
Grubbs et al.~\cite{grubbs2018pump},
Lacharit\'{e} et al.~\cite{lacharite2018improved} and Grubbs et al.~\cite{grubbs2019learning}. These works exhibited database reconstruction attacks in scenarios where
range queries are made to an \emph{encrypted} database and
the access pattern (i.e.~which records are returned) \cite{kellaris2016generic, lacharite2018improved} or communication volume (i.e.~the number of records returned)~\cite{kellaris2016generic, grubbs2018pump} is observed by the malicious server. 
 %In this work, we assume the victim VM executes range queries on the private database 
 %Grubbs et al.~\cite{grubbs2018pump} shows such an attack in an ideal case where the attacker can gain the exact value of the volumes whereas we consider the case where the noisy value of the volumes are leaked. 
However, recall that in our threat model, an attacker cannot simply observe the access pattern or communication volume, 
and must instead resort to side channels 
(such as a shared cache) to learn information.
 %Indeed, since our threat model is weaker, we must show how to obtain information on the communication volume through side-channels alone.
 %We exhibit an attack wherein the spy VM exploits the cache-side channel to estimate the volumes of range queries made to the private database. 
 Indeed, our attack will utilize the cache side-channel to learn
 information about the communication volume of the range queries.
 Briefly, this is done by finding a line of code that is executed once for each record returned in a response to a range query, 
 and tracking how many times that line of code is executed.% by the victim yields the volume of the response. 
 
 Since cache side-channels are inherently noisy, we are only able to measure the \emph{approximate} or \emph{noisy} volumes of the range queries.
 We emphasize that even adding a small amount of noise to the volume of each range foils the
 reconstruction attacks from prior work.
 We assessed the effects of noise
 on brute force reconstruction (an analogue of the brute force algorithm suggested by~\cite{kellaris2016generic} for the dense database setting), and on the clique-finding approach developed by~\cite{grubbs2018pump}. 
 As will be discussed in depth in Section~\ref{sec:ourcontrib}\anote{here}, we conclude that both of these approaches fail in the noisy setting.
 
 \iffalse
 \dnote{fill in}
 Indeed, using the data obtained from running our cache attack on a database of size ***, a brute force reconstruction failed to find any candidate database after a day of running, due to the fact that the added noise means that there are exponentially more possibilities to check.
 \dnote{I really want to write something here about the previous approaches failing
 in the case of noisy volumes, but I don't know if we have the experimental data to support this!!}\anote{added a note}\lnote{needs more work.}
 
 %\dnote{Next sentence is possibly misleading
 %about what this paper is about...}
 %In this work, we assess the effectiveness of previous algorithms
 %in the ``noisy'' setting and
 %develop new algorithmic approaches to solve the problem of database reconstruction from ``noisy'' volumes.
 
 %\dnote{This is now repetitive. Removed it for now.}
 \iffalse
 We find that
 a modification of the brute-force-search approach of~\cite{kellaris2016generic} to the dense setting fails in the ``noisy setting'' and does not succeed in recovering any candidate solution within a reasonable running time.
 We therefore focus on comparing the clique-finding algorithm based on the approach of ~\cite{grubbs2018pump} with our own newly developed algorithms for the noisy setting.
 
 \fi
 
 \dnote{Need to add something here about how regular (non-noisy) clique-finding failed, but that we are still inspired by their techniques.}
 \fi
 
 %\vspace{-3mm}
 
 \paragraph{Our approach.}
 We develop a new algorithmic approach that reduces our noisy problem to other computational problems that are well-studied in the literature and for which highly optimized solvers have been developed.
 Specifically, we will leverage both
 a noise-tolerant clique-finding algorithm (similar to \cite{grubbs2018pump}, but with some crucial modifications) as well as a closest vector problem (CVP) solver.
 In more detail, we first use the noisy cache data to craft an instance of the clique-finding problem that is noise-tolerant. Recovered cliques will then be used to obtain candidate databases that are ``close'' to the original database. To extrapolate volumes that may be entirely missing from the recovered cliques,
 we develop a ``Match \& Extend'' algorithm. After the Match \& Extend step,
 we expect to have reconstructed approximate volumes for all ranges.
 We then apply a ``Noise Reduction Step'' that takes the ``close'' solution outputted by 
 the previous step, consisting of approximate volumes for each
 of the ranges $\range{i}{i}$ for $i \in N$,
 and uses it to craft an instance of the CVP problem. Solutions to the CVP problem correspond to reconstructed databases in which the overall noise is further reduced.
 %, as we discuss in detail in the experimental section, we ultimately obtain a reconstructed database with average error of $0.22 \%$ or less.

We note that since our side-channel attack proceeds by measuring (approximate) range query volumes, 
it is agnostic to whether the victim's database is encrypted. As long as the spy can
monitor a line of code that is executed by the database engine for each record returned
by a range query, our attack is feasible.
Searchable encryption schemes that have this property would still be susceptible to this side-channel attack. 
For example searchable encryption schemes that can be integrated with standard database engines, such as order preserving encryption~\cite{SIG:AKSX04,EC:BCLO09} and order revealing encryption~\cite{EC:BL0SZZ15}.

 
 A limitation of our work is that our approach uses solvers for NP-hard problems as subroutines. The complexity of these NP-hard problems grows
 quickly \dnote{exponentially?}
 with the \dnote{square of the} size of the range, and therefore will work well in practice for ranges up to size 15. This is in contrast to the recent work of Grubbs et al.~\cite{grubbs2019learning}, which showed how to do ``approximate reconstruction'' in a way that scales only with the desired accuracy level and not the range size.
 However, the work of Grubbs et al.~\cite{grubbs2019learning} assumes the adversary gets to perfectly observe the \emph{access pattern}---i.e. which records are returned for each query---which provides far more information than simply observing the volumes. It seems difficult to extract the \emph{access pattern} for a
 %information about which individual records are returned in 
 response to a database query from a cache side-channel attack.\footnote{To extract access pattern from the cache, Prime \& Probe must be used to monitor the data cache, and because a single record from the database can fill a large portion of the cache, it is difficult to distinguish which records were accessed by observing only the cache. Additionally, the mapping from the memory location to cache line is not one to one and hence, a large number of records will map to the same cache locations, making it difficult to distinguish which records were accessed.
 %\footnote{Since to extract a meaningful access pattern, Prime \& Probe instead of Flush+Reload must be used to monitor the data cache, and because a single record from the database can fill a large portion of the cache, it is difficult to distinguish which records were accessed by observing only the cache. Additionally, the mapping from the memory location to cache line is not one to one and hence, a large number of records will map to the same cache locations, making it difficult to distinguish which records were accessed.
 %This is because Prime \& Probe instead of Flush+Reload must be used when monitoring the data cache, and due to the fact that a single record from the database can fill a large portion of the cache, which makes it difficult to distinguish which records were accessed by observing only the cache. Additionally, the mapping from the memory location to cache line is not one to one and hence, a large number of records will map to the same cache locations, making it difficult to distinguish which records were accessed.
 }
%\anote{following should be filled}


We extensively test our attack in various scenarios, using real databases (with data distribution close to uniform), as well as synthetic databases with Gaussian data and various settings of the standard deviation. We also experiment with uniform queries (each possible range query is made with equal probability) and non-uniform queries (different range queries are made with different probabilities). We also extend our analysis to study the effect of extra load on the system. Furthermore, we extend the Match \& Extend algorithm by studying what will happen if not all the possible ranges are queried. 
%In each setting, we show that our attack is practical for databases of size up to $100,000$ and ranges of size up to $12$. We achieve an average error rate of $\newnote{} \%$ or less in each setting.


\iffalse
Cloud computing has gained much attention in the last decades, and clouds are handling more services. \anote{I want to talk about IOT as well since the size of the database were are attacking is rather small, so it fits the setting}. Another service on the rise is Intern of Things which is being utilized more often in everyday life. In both of these services, security plays an essential role for both the designer and the user of the system. These area has attracted a significant amount of attention from the academic community which shows their weakness and ways to improve them. On the other hand, side channels attacks have shown to be effective in both of these settings. Attacks such as cache side-channel attacks and power analysis are just two examples of attacks which are shown to be effective in the cloud computing environment and IOT environment, respectively. These attacks use the information which is not directly accessible to the attacker, but by being ``close'' to the victim, the attacker can gain useful knowledge about the status of the victim and mount a successful attack as a result. Most of the work in this area focused on Crypto Libraries and trying to extract secret information of the victim. However, our goal in this work is to show yet another side-channel attack but on the typical data processing software which has not been explored as much. Hence, we show an attack on SQLite, which is widely used in practice. SQLite is a C-language library that implements a small and fast SQL database engine. SQLite is among top ten databases in the ranking released by db-engines.com.
%\dnote{Add some stats on usage of SQLite.}
%\dnote{By the above, I meant to include stats on the number of people using SQLite in practice.}
\\
\fi

%\vspace{-3mm}

\paragraph{Formal setting.} We consider a database of size $n$ and an attribute with range size $N$ for which range queries (i.e.~SQL queries that return all records corresponding to values between $[a,b]$) can be made. The size of query response corresponding to range query $\range{a}{b}$ is denoted by $\size{\range{a}{b}}$ and, similar to Grubbs et al.~\cite{grubbs2018pump}, the volumes in the form of $\range{1}{i}$ for $1 \leq i \leq N$ are called ``elementary volumes''. Note that to fully recover all the ranges in the form $\range{i}{i}$ it is enough to recover ``elementary volumes''. 
In this paper each volume is represented by a node in a graph. A node with label $v_i$ correspond to a range of volume $v_i$.
In this paper we refer to each node of the graph by its label.  The goal of our attack is to reconstruct the entire column corresponding to the field with range size $N$. Specifically, for each $i \in [N]$, we would like to recover the number of records $n_i$ that take value $i$ in the attribute under inspection. The focus of this work is on ``dense'' databases, meaning that every possible value from $1$ to $N$ is taken by some records in the database.\footnote{We note that in the searchable encryption setting this is not the typical case since ciphertexts encrypting values between $1$ and $N$ are typically sampled from a larger space. However, in this work, our main focus is on cleartext databases and attackers who learn information about them via the cache side-channel.} For simplicity, we assume that ranges are always from $1-N$. However, the result generalizes to any range $a-b$, where database records can take on at most $N$ discrete values within the range.
\iffalse
The reconstruction problem has been studied in several recent papers~\cite{kellaris2016generic, grubbs2018pump} \dnote{citations missing.}. Motivated by settings in which the server itself is malicious, the attack model in those papers assumes that the attacker receives all volumes corresponding to all range queries made to the database in the clear. 
Grubbs et al.~\cite{grubbs2018pump} mentioned that an attacker who is intercepting the connection between user and server can count the TLS packets in order to obtain the volumes of range queries, but did not consider the difficulties that arise when the measurement channel introduces noise into the computed volumes.
\fi
%\dnote{The Pumping up the Volume paper mentions some stuff about getting the volume by counting the number of TLS packets. But this seems like it would be hard to get an exact count from this type of data and so the volumes would be noisy as in our setting. It doesn't seem like they actually tried the attack. We should say the above in a tactful way.}
Our attack model assumes that a malicious party can only launch side-channel attacks to reconstruct the database. In particular, we assume that the attacker monitors its read timing from a cache line to deduce useful information about the victim. As discussed, the noise introduced by the cache side-channel makes our setting more challenging.\footnote{We note that Grubbs et al.~\cite{grubbs2018pump} mentioned a type of side-channel where an attacker intercepts the connection between user and server and counts the TLS packets in order to obtain volumes of range queries, but they did not consider the difficulties that arise when the measurement channel introduces noise into the computed volumes.}
%This setting makes the problem harder. \dnote{Aria: please put in more details on the attack setting.}\anote{done}\\

\iffalse
%\dnote{Should the following be removed?}
\textbf{Motivating example:} 
\dnote{Replace the following with an example from our real
datasets.
E.g.; a database can store details of all sales made by some company in a given calendar year. The database includes a field that indicates which month each sale was made in. Thus, this field has range $[1-12]$ and range queries would correspond to returning all sales that were made within a range of months. Successful reconstruction of this field implies \emph{learning how many sales were made each month} which could potentially be private information that the company does not want to release.}\anote{I am not sure if we want to have the example or just the citations?} There has been great amount of work in this area~\cite{kellaris2016generic, grubbs2019learning, lacharite2018improved, kornaropoulosdata} on  encrypted databases and ~\cite{grubbs2018pump} on normal databases.\dnote{Maybe just pointing to papers that studied the reconstruction problem under a different threat model is enough and we don't need the motivating example.}\anote{done}\\


\dnote{Remove this?}
\textbf{Connection with differential privacy:} 
\dnote{Aria, I would really like to see you write this paragraph in an organized, logical, convincing way. Before writing please write a list of bullet points that you want to address in this paragraph and send to me.}
It is shown in~\cite{kellaris2016generic,grubbs2018pump} how to reconstruct the database given the volume of range queries. Kellaris et al.~\cite{kellaris2017accessing} shows a construction for databases which can support range, point, and attribute queries and they proved it achieves differential privacy if the noise is drawn from Laplace distribution with specific parameters. The previous works motivated us to consider the cases where the volume are perturbed according to some Laplacian distribution. 
\anote{continue here}
\fi

\iffalse
\anote{point to be addrressed in this paragraph}
\begin{itemize}
    \item Complete Reconstruction of the database by leaking exact volumes as shown by Grubbs as well as Kellaris 
    \item Kellaris in different paper showed a countermeasure against previous attack by adding noise to the volume which is seen by attacker
    \dnote{I would add here that their countermeasure provably achieves differential privacy, under sufficient noise drawn from an appropriate distribution.}
    \item motivated by the previous work which is in differential privacy setting, we asked the question: What will happen if the volumes are perturbed according to some Laplacian distribution. How resilient our attack is in this case?
    \item \dnote{And what did we conclude? Put in something like: for low levels
    of noise our attack remains effective. Or whatever is supported by the experimental data.} 
\end{itemize}
\fi

\iffalse
The main question answered by differential privacy is how to release accurate statistical information about a database but at the same time preserving the privacy of each individual. One major attack~\cite{narayanan2008robust} demonstrate a de-anonymization technique which by having only a small amount of extra knowledge about each subscriber can reveal their records in the dataset. One way to defends against such an attack is to introduce a small amount of noise to each entry as shown in~\cite{dwork2006calibrating}. We focus on this type of countermeasure in this work as well and measure the performance of our algorithm given that a small amount of noise is added to our measured values. 
\dnote{Aria: Please fill this in.}\anote{differential privacy need two sided-distribution... relation to us?!}\\
\fi

\subsection{Our Contributions}\label{sec:ourcontrib}
%\dnote{The following is just a sketch. Needs to be filled in and fleshed out. May not appear as a bulleted list in the final version.}

We next summarize the main contributions of this work.

%Summary of our contributions:
\textbf{Weaker threat model: Side-channels.} Prior work considers a threat model of a malicious server that is computing on an encrypted database. We consider an honest server computing on a cleartext (or encrypted) database and a malicious third-party that is co-located with the honest server in the cloud, sharing a cache, and cannot issue queries to the database. The malicious third-party can only obtain information by monitoring the shared cache. In particular, this means that the third-party cannot learn the \emph{exact} volumes of range queries and only obtains \emph{approximate} or \emph{noisy} volumes.



\textbf{Assessing effectiveness of
previous algorithms in the noisy setting.}
We first analyzed the effectiveness of a brute force attack,
similar to the one suggested in the work of Kellaris et al.~\cite{kellaris2016generic}, but adapted to the \emph{noisy}
and \emph{dense} database setting.
%A brute force attack for a uniform query distribution and a noiseless setting works as follows: The attacker obtains a good approximation of the probability of each volume being returned, which we call the ``base probability list''. In the next step of the algorithm the attacker computes the ``candidate probability list'' by trying all potential values for each entry in the database and comparing the ``candidate'' with the ``base'' and then picks the result which is closest to the ``base''. To construct the ``base probability list'' from the noisy volumes, since each volume is approximately close to the correct volume, for each noisy volume we create a range of acceptable volumes. \dnote{I do not understand.}\anote{for future edit here.....} The rest of the algorithm works similar to noiseless case.  \dnote{How is this adapted to the noisy setting?}\anote{tried to answer}
When we ran this version of the brute-force search algorithm, it failed to return a result, even after a day of running. 
We expected this to be the case, since when the volumes are noisy, there are far more choices that need to be checked in each step of the brute force search.
%\dnote{Can you be more specific. How long did you let it run?}\anote{commented out the next part}
%\dnote{***Some explanation here???*** E.g. runs longer than the noiseless case because in each step of the brute force search there are far more choices.}
%, in the cases where the volumes are noisy and the range of the values are large \dnote{Can you be more specific?}\anote{here}. 

We next analyzed the effectiveness of an attack based on clique-finding, as in the work of Grubbs et al.~\cite{grubbs2018pump}.
%The second algorithm is to construct a graph from the data and run a clique-finding algorithm on it. To construct the graph from the exact volumes, one first creates nodes with labels corresponding to their volume, i.e. the node with label $v_i$ has volume $v_i$. There is a connection between node $v_i$ to $v_j$ if there exists a node $v_k$ such that $v_i = v_j + v_k$. 
A graph is constructed based on the observed volumes of the range queries.
To construct the graph from \emph{exact} volumes, one first creates nodes with labels corresponding to their volume, i.e. the node with label $v_i$ has volume $v_i$. There is a connection between node $v_i$ to $v_j$ if there exists a node $v_k$ such that $v_i = v_j + v_k$. Note that by this construction the nodes corresponding to elementary volumes form a clique of size $N$ which can be recovered by clique finding algorithm. 
The ranges $\range{1}{1}, \range{1}{2}, \ldots, \range{1}{N}$ and the full database can then be recovered from this information.

%, i.e. nodes that are corresponds to the ranges of the form $\range{1}{i}$ for $1 \leq i \leq N$ form a clique. 
%So a clique finding algorithm returns a clique of size $N$, from which the full database can be recovered. 
In the noiseless setting we always expect to get a clique of size $N$; however, in the noisy setting there are multiple edges missing
in the constructed graph and so a clique of size $N$ will typically not exist.
%because the mentioned equality is not satisfied in the majority of cases since the volumes are noisy. 
For example, when we ran the algorithm on our noisy data with $N = 12$, the size of the cliques returned was at most $3$. 
Further, the clique of size $3$ no longer corresponds to the volumes of the elementary volumes,
%defined in Grubbs et al.~\cite{grubbs2018pump}
and therefore is not useful for (even partial) reconstruction of the database.
%A clique of size $3$ is not useful for reconstruction as there are multiple ranges which can form clique of $3$ and combining all of them to recover the database is not feasible. 


%The approaches mentioned in the previous worked failed to work in the noisy case. 
%As we will show our algorithm that is a variant of the clique finding algorithm with recursive procedure for the noisy cases.



\textbf{Developing algorithms for the noisy setting.} 
%\dnote{This needs to be rewritten.}\anote{tried to address it}
%~\cite{grubbs2018pump} 
%We suggest new algorithms for the noisy setting and compare their performance with the clique-finding approach.
%This involves several steps:
 %   \begin{itemize}
 %       \item 
Whereas Grubbs et al.~\cite{grubbs2018pump} used exact volumes to reduce the database reconstruction to a clique-finding problem, we begin by reducing the reconstruction problem given with volumes to a \textbf{Noise-Tolerant Clique Finding Problem} by introducing a notion called a \emph{noise budget}. 
%The cases in which the exact volumes are leaked are captured by having a \emph{noise budget} equal to $0$. 
%To construct the graph from \emph{exact} volumes, one first creates nodes with labels corresponding to their volume, i.e. the node with label $v_i$ has volume $v_i$. 
Remember in the \emph{exact} volume case, there is a connection between node $v_i$ to $v_j$ if there exists a node $v_k$ such that $v_i = v_j + v_k$. 
Here, to construct the graph from \emph{noisy} volumes, we create a window, $w(v_k)$, of acceptable values around each leaked volume $v_k$, where the width of the windows is determined by the noise budget. We place an edge between node $v_i$ and $v_j$ if there exists a node $v_k$ such that $| v_i - v_j | \in w(v_k)$. 
The clique finding algorithm will return a clique that allows one to recover the volumes,
%of the ranges $\range{1}{1}, \range{1}{2}, \ldots, \range{1}{N}$ 
and the full database can then be recovered from this information. 
An attacker can determine a good setting of the \emph{noise budget} by mounting an attack in a preprocessing stage on a different, known database under same or similar conditions.
Specifically, the attacker can first create its own known database (unrelated to the unknown private database). The attacker can then simulate the side-channel attack on the known database on a similar system and compare the recovered approximate/noisy volumes with the correct volumes, and observe by how much they are off, to determine an appropriate \emph{noise budget}.
%to assess the quality of observed traces, allowing a good guess for the noise budget.
%The attacker can then simulate the side-channel attack on the known database and compare the approximate/noisy volumes recovered with the correct volumes and observe by how much they are off, to determine an appropriate \emph{noise budget}. 
In some cases, incorporating the \emph{noise budget} into the construction of the graph and running the clique-finding algorithm already allows us to successfully reconstruct a fairly accurate database. However, there are some cases where, even after increasing the \emph{noise budget}, the algorithm fails to recover a candidate database (i.e.~a clique of size $N$ does not exist).
Further, even in cases where increasing the \emph{noise budget} does allow for reconstruction of some candidate database, the accuracy of the candidate database suffers and the run-time increases. We therefore introduce an additional algorithm called \textbf{Match \& Extend}, which allows successful reconstruction of candidate databases with improved accuracy.
 
 The \textbf{Match \& Extend} algorithm starts by obtaining a candidate clique from the graph. If the size of the clique is equal to $N$ (the maximum range) we are done. Otherwise, the algorithm looks at all the other cliques present in the graph starting from the largest to the smallest. For each clique, a potential database is recovered. We then pick one of the databases as our base solution and compare it with the other recovered databases. In the \textbf{Match} phase, the algorithm looks for the ``approximate longest common substring'' between two databases. The ``approximate'' version of the longest common substring considers two substrings equal if their corresponding values are within an acceptable range dictated by the \emph{noise budget}. Two values $a$ and $b$ are ``approximately'' equal if $ | a - b | \leq \min(a,b) \cdot 2 \cdot \texttt{\small noise budget}$. Then for the databases which have enough overlap with the base solution, the \textbf{Extend} phase will compare the non-matching parts of the two solutions and will try to reconcile the volumes in them into one ``combined'' database.
        
        % break any large value in the base solution with the help of the candidate database, it also add missing values to the database.  
        
%       \item 
Finally, in the \textbf{Noise Reduction Step}, we use the results of the previous steps along with a closest vector problem (CVP) solver to reconstruct nearly the \emph{exact} original database, despite the noisy measurements. The recovered database of the previous step returns the ranges of the format $\range{1}{1}, \range{2}{2}, \ldots, \range{N}{N}$. We can reconstruct potential volumes for each range with these recovered volumes and for each computed volume we select the closest volume from the initial noisy volume set obtained from the side-channel data. We construct a lattice basis using the known linear dependencies between the volumes of different ranges. The volumes obtained from the side-channel data correspond to the target point for the CVP problem. Using the CVP solver, we find a set of volumes contained in the lattice (so they satisfy the linear dependencies) that are closest to the target point. This ``self-correction'' technique allows us to recover a better candidate solution for the database. 
        
        %\item %Whereas~\cite{grubbs2018pump} used clique-finding, We begin by reducing the reconstruction problem (given exact, non-noisy volumes) to a subgraph isomorphism problem. A solution to the subgraph isomorphism instance 
        %allows us to yields a mapping of \emph{all} ${N \choose 2} + N$ possible ranges to corresponding volumes. In particular, this allows us to reconstruct the volumes corresponding to the ranges
        %isolates the volumes that correspond to the ranges $[1-1], [2-2], \ldots, [N-N]$.
        %out of the set of ${N \choose 2} + N$ values corresponding to all ranges. Reducing to subgraph isomorphism (a more general problem) instead of clique-finding allows us to encode \emph{auxiliary information} into the problem instance, as will be discussed later. Moreover, the solution of the subgraph isomorphism instance yields a mapping of \emph{all} ${N \choose 2} + N$ ranges to volumes, whereas a solution to the clique instance yields a mapping of the ``elementary'' ranges ($[1-1], [1-2], \ldots, [1-N])$) to corresponding volumes. While in the noiseless case, the full mapping can be recovered given the mapping of the elementary ranges, this is not the case in the noisy setting. Furthermore, we require the full mapping obtained by the subgraph isomorphism solver to construct an appropriate CVP instance, as discussed below.
        %\item \dnote{Is this still correct? Do our experiments support this? Please re-write so that it is accurate.} We develop techniques for creating a subgraph isomorphism instance from the noisy data obtained from the cache. Specifically, our cache data will include multiple candidate volumes corresponding to each range query. Experimental results show that we can include all the candidate volumes in the problem instance and still obtain solutions that are fairly close to the original database.
        %while still maintaining high success probability. This is in contrast to polynomial factorization, exhaustive search or clique-finding that were used in previous works. \dnote{need experimental results to show that subgraph isomorphism is more resilient to noise than the other techniques.} This means that using our cache data, we can successfully reconstruct multiple candidates for the volumes of all ${N \choose 2} + N$ ranges. However, due to the fact that the volume measurements obtained from the cache are noisy, even for ``good'' candidate solutions, each volume will only be within $\pm c$ of the correct solution, where $c$ is the accuracy of the volumes obtained by the side-channel attack.
        %\item We use the results of the subgraph isomorphism solver along with a closest vector problem (CVP) solver to reduce the noise further and reconstruct nearly the \emph{exact} original database, despite the noisy measurements. We emphasize that even if the correct volumes corresponding to the ranges $[1-1], [2-2], \ldots, [N-N]$ are not present in the solution of the subgraph isomorphism instance, using our CVP solver we can still reconstruct (almost all) the correct volumes corresponding to $[1-1], [2-2], \ldots, [N-N]$, such that only a small number of volumes (typically $1$ to $3$ volumes out of $15$) are off by $\pm 1$.
        %We also develop a technique that ensures that the dimension of the CVP instance remains low as the size of the range grows.
        %\item We also consider settings where auxiliary information about either the query distribution or the data distribution is known. We show that auxiliary information about the query distribution can be used to construct subgraph isomorphism instances with fewer nodes and that auxiliary information about the data distribution can be encoded into the subgraph isomorphism instance itself. Both of these techniques significantly  improve the quality of the obtained solutions, allowing us to extend our database reconstruction attacks to further regimes.\dnote{Fill in a short description of how we incorporate the auxiliary information.}
%    \end{itemize}


\textbf{Launching the side-channel attack.} 
We adapt the Flush+Reload technique for obtaining the (approximate) volumes of responses to range queries in SQLite. This allows us to learn a set of \emph{noisy} volumes corresponding to the range queries made by external parties to the database stored by the victim. The monitoring process starts as soon as an activity is detected and continues for the duration of the SQLite query processing. Since the databases we attack are large, the processing takes an extended amount of time, meaning that there are many opportunities for noise to be introduced into a trace. On the other hand, we require accurate measurements for our attack to succeed.\footnote{Similar to keystroke timing attacks of Gruss et al.~\cite{gruss2015cache}}
We contrast our setting to other side-channel settings, which typically require \emph{accurate} measurements over a \emph{short}
period or, can tolerate \emph{ inaccurate} measurements over a \emph{longer} period.
For example, side-channel attacks on cryptographic schemes require accurate information to reconstruct the high-entropy keys, but typically take a short period of time, since the keys themselves are short. On the other hand, side-channel attacks for profiling purposes typically monitor an application for longer periods of time, but can tolerate noise well since their goal is just to distinguish between several distinct scenarios.

To achieve high accuracy over a long period of time, we must handle interrupts as well as false positives and false negatives. For interrupts, we must mitigate their effects by detecting and dropping those traces in which an interrupt occurs. There can also be false positives as a result of CPU prefetching, which we show how to detect.
False negatives occur if the victim process accesses the monitored line of
code after the spy ``Reloads'' the line, and before the spy
``Flushes'' the line.
We do not directly detect false negatives, but instead show how to deal with them algorithmically.

%\vspace{-3mm}
\subsection{Overview of Experimental Results} 
We ran our attacks in five different experimental settings including uniform and non-uniform queries on real databases and synthetic databases which were sampled from Gaussian (Normal) distributions with different standard deviations as well as in two sets of experiments where the system is under heavy load and other cases where some of the range queries are missing. The databases all contained $100,000$ rows with $135$ attributes. The synthetic database from the Gaussian distribution has the same number of entries and attributes, but the column on which the range queries are made is sampled from Gaussians with standard deviation of $3$ and $4$, which represent narrow and wide Gaussians, respectively. The Match \& Extend algorithm recovered the database in $100 \%$ of the cases within $190$ seconds with maximum error percentage of $0.11 \%$.
%\newnote{confusing as pointed out by reviewer.}

\dnote{Just give the bottom line here...}\anote{fixed}
\iffalse
In Section~\ref{sec:experiments}, we define a quantity called error percentage which roughly shows how ``close'' the recovered database is to the actual one. We show that by increasing the noise budget in the noise-tolerant clique finding problem we can recover the databases in most but not all of the experiments. However, by fixing the noise budget and using the Match \& Extend algorithm we can recover all of the databases more efficiently. Additionally, the error percentage of the recovered answers in Match \& Extend is better than that for noise-tolerant clique finding problem. Finally, we assess the effectiveness of noise reduction step, and conclude that by using that we can enhance the accuracy of the recovered databases further. For example for the scenario the scenario involved real database and uniform query, we showed that the average of maximum error percentage is $0.86 \%$ for noise-tolerant clique finding but it will reduce to $0.22 \%$ by using the Match \& Extend algorithm and further reduces to $0.20 \%$ by using noise reduction step.
\fi

\anote{a paragraph here on the experimental result, final algorithm, our algorithm managed to recovered 100 percents to within 0.01 accuracy. Report the final Match \& Extend, maybe not the other attacks scenarios}

\dnote{Quick recap of when our attacks succeed.}
\dnote{Should discuss here what exactly are the requirements on the query distribution, and how our requirements compare to those of prior work.}
%We discuss our experimental results in more detail in the following section.

%\subsection{Overview of Experimental Results}
%\anote{here...}

\subsection{Related Work}
\textit{Cache Attacks} were introduced by Tsunoo et al.~\cite{tsuno_cache} that shows a timing attack on MISTY1 block cipher.
Later, Osvik et al.~\cite{osvik2006cache} presented an attack that allowed the extraction of AES keys. In another early work, Ac\i i{\c{c}}mez~\cite{aciiccmez2007yet} showed an attack that targets instruction cache.
%to extract the information of whether the multiplication function is called or not.
Ristenpart et al.~\cite{ristenpart2009hey} demonstrated the possibility of launching cache side-channel attacks in the cloud (as opposed to on a local machine) and they pointed out that such vulnerabilities leak information about the victim VM. Subsequent work showed how the cache side-channel can be used to extract cryptographic keys for ElGamal~\cite{zhang2012cross}, AES~\cite{irazoqui2014wait}, RSA~\cite{184415} and recently BLISS~\cite{bruinderink2016flush} (a lattice-based signature scheme).
%\textit{Cache Attacks} are a powerful tool that proved to be useful in extracting secret information from victim programs. In one of the early works, Osvik et al.~\cite{osvik2006cache} presented one of the first practical attacks against an AES implementation based on a T-table. They used a Prime \& Probe attack by filling a cache, letting the victim run and then measuring the access time to each cache set. 
%In another early work, Ac\i i{\c{c}}mez~\cite{aciiccmez2007yet} showed an attack that targets instruction cache to extract the information of whether the multiplication function is called or not. 
In more recent work, Yarom and Falkner~\cite{184415} presented a powerful attack using Flush+Reload on the Level 3 cache of a modern processor. They tested their attack in two main scenarios, (a) victim and spy running on two unrelated processes in a single operating system and (b) victim and spy running on separate virtual machines. Another attack of note by Yarom and Benger~\cite{yarom2014recovering} on ECDSA leaks the nonce which results in signature forgery. 
%As a result of this leakage, the attacker gains access to the private key and can forge as many signatures as desired. 
A recent work by Moghimi et al.~\cite{moghimi2017cachezoom} showed the vulnerability of AES encryption in an SGX environment which, prior to this attack, was broadly believed to be secure. 
Ge et al.~\cite{ge2018survey} surveyed recent attacks and classified them according to which shared hardware device they target. Yan et al.~\cite{telepathy} shows the effectiveness of Flush+Reload and Prime \& Probe to reduce the search space of DNN architectures. In a more recent type of attack, Hong et al.~\cite{cacheNNFingerprint} shows how to perform Deep Neural Network fingerprinting by just observing the victim's cache behavior. 
In another work by Hong et al.~\cite{Hong2020How}, it is shown how to use cache attack to construct the main components of the Neural Network on the cloud.
%\dnote{Should we cite Spectre and Meltdown? Compare our threat model to theirs?}\anote{I believe these two papers are less relevant to us}

\textit{Database Reconstruction} 
Kellaris et al.~\cite{kellaris2016generic}, motivated by practical implementations of searchable symmetric encryption or order-preserving encryption, studied the effect of auxiliary information on the overall security of the scheme. They identified two sources of leakage (a) access pattern (b) communication volume. They developed a reconstruction attack in which the server only needs to know the distribution of range query. They presented an attack using $N^4$ queries, where $N$ is the ranges of the value. Lacharit{\'e} et al.~\cite{lacharite2018improved} presents various types of attacks: full reconstruction, approximate reconstruction as well as a highly effective attack in which adversary has access to a distribution for the target dataset. Their attacks are based on the leakage of access pattern as well as leakage from the rank of an element. Grubbs et al.~\cite{grubbs2018pump} present an attack that reconstructs the database given the volumes of the response of range queries. They showed an attack using a graph-theoretic approach and specifically clique finding. Each volume is presented with a node in the graph. They demonstrated properties that hold in practice for typical databases and based on these properties they developed an algorithm which runs in multiple iterations of adding/deleting nodes. 
%At each iteration either some nodes are removed from the graph or added to the graph. 
Once there is no more addition and deletion to be performed they announce that as the candidate database. They showed that this approach is indeed successful in recovering most of the columns of their example database. In cases where this algorithm could not find any possible result they used a clique algorithm to reconstruct the database, and they showed that clique could help to reconstruct even more instances.

In another line of work regarding searchable encryption, Cash et al.~\cite{cash2015leakage} presented leakage models for searchable encryption schemes and presented attacks. Specifically using this leakage they could recover queries as well as the plaintext. Naveed et al.~\cite{naveed2015inference} presented a series of attacks on Property-preserving Encrypted Databases. Their attack only used the encrypted column and used publicly known information. They showed an attack which could recover up to a certain attribute for up to $80\%$ of users. Grubbs et al.~\cite{grubbs2017leakage} presented an attack on order-preserving encryption and order-revealing encryption and showed they can reveal up to $99\%$ of encrypted values. Kornaropoulos et al.~\cite{kornaropoulos2019data} studied the database reconstruction given leakage from the $k$-nearest neighbours ($k$-NN) query. 
%Specifically, they first presented the feasibility of ``exact reconstruction'' and further presented a practical attack for ``approximate reconstruction''. 
In a follow up work by the same authors, Kornaropoulos et al.~\cite{kornaropoulos2020state} extended their previous work by presenting an attack on encrypted database without the knowledge of the data or query distribution. All these attacks are in the encrypted database setting in which each value is encrypted whereas the focus of this work is on databases where the value of each entry is saved in clear text, and an attacker who may only obtain information about the database via side channels.
\dnote{are we missing important citations on attacks on searchable encryption?}









==> backup.tex <==

\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. Please do not use it for A4 paper since the margin requirements for A4 papers may be different from Letter paper size.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as Ò3.5-inch disk driveÓ.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ÒWb/m2Ó or Òwebers per square meterÓ, not Òwebers/m2Ó.  Spell out units when they appear in text: Ò. . . a few henriesÓ, not Ò. . . a few HÓ.
\item Use a zero before decimal points: Ò0.25Ó, not Ò.25Ó. Use Òcm3Ó, not ÒccÓ. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use Ò(1)Ó, not ÒEq. (1)Ó or Òequation (1)Ó, except at the beginning of a sentence: ÒEquation (1) is . . .Ó

\subsection{Some Common Mistakes}
\begin{itemize}


\item The word ÒdataÓ is plural, not singular.
\item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ÒoÓ.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ÒinsetÓ, not an ÒinsertÓ. The word alternatively is preferred to the word ÒalternatelyÓ (unless you really mean something that alternates).
\item Do not use the word ÒessentiallyÓ to mean ÒapproximatelyÓ or ÒeffectivelyÓ.
\item In your paper title, if the words Òthat usesÓ can accurately replace the word ÒusingÓ, capitalize the ÒuÓ; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ÒaffectÓ and ÒeffectÓ, ÒcomplementÓ and ÒcomplimentÓ, ÒdiscreetÓ and ÒdiscreteÓ, ÒprincipalÓ and ÒprincipleÓ.
\item Do not confuse ÒimplyÓ and ÒinferÓ.
\item The prefix ÒnonÓ is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ÒetÓ in the Latin abbreviation Òet al.Ó.
\item The abbreviation Òi.e.Ó means Òthat isÓ, and the abbreviation Òe.g.Ó means Òfor exampleÓ.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if you filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named ÒHeading 1Ó, ÒHeading 2Ó, ÒHeading 3Ó, and ÒHeading 4Ó are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation ÒFig. 1Ó, even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity ÒMagnetizationÓ, or ÒMagnetization, MÓ, not just ÒMÓ. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write ÒMagnetization (A/m)Ó or ÒMagnetization {A[m(1)]}Ó, not just ÒA/mÓ. Do not label axes with a ratio of quantities and units. For example, write ÒTemperature (K)Ó, not ÒTemperature/K.Ó

\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.



\begin{thebibliography}{99}

\bibitem{c1} G. O. Young, ÒSynthetic structure of industrial plastics (Book style with paper title and editor),Ó 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15Ð64.
\bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
\bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
\bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
\bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
\bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
\bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
\bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
\bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
\bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
\bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
\bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
\bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
\bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
\bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
\bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
\bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
\bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
\bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
\bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 






\end{thebibliography}


